Analysis of Deep Learning-Based Colorization and Super-Resolution Techniques for Lidar Imagery

Modern lidar systems can produce not only dense point clouds but also 360 degrees low-resolution images. This advancement facilitates the application of deep learning (DL) techniques initially developed for conventional RGB cameras and simplifies fusion of point cloud data and images without complex processes like lidar-camera calibration. Compared to RGB images from traditional cameras, lidar-generated images show greater robustness under low-light and harsh conditions, such as foggy weather. However, these images typically have lower resolution and often appear overly dark. While various studies have explored DL-based computer vision tasks such as object detection, segmentation, and keypoint detection on lidar imagery, other potentially valuable techniques remain underexplored. This paper provides a comprehensive review and qualitative analysis of DL-based colorization and super-resolution methods applied to lidar imagery. Additionally, we assess the computational performance of these approaches, offering insights into their suitability for downstream robotic and autonomous system applications like odometry and 3D reconstruction.

==> algs/al_kf.tex <==
\begin{algorithm}[t]
    \footnotesize
	\caption{UAV tracking fusing signal images and point clouds} 
	\label{alg:fusing_data}
	\KwIn{ \\
	    \vspace{.42em}
	    \hspace{.5em}Raw pointcloud:  $\mathcal{P}_{raw}^t$ \\
                  
	    \vspace{.23em}
	    \hspace{.5em}Signal image:  $\mathcal{S}^{t} $ \\

            \vspace{.23em}
	    \hspace{.5em}Target UAV point cloud:  $\mathcal{P}_{UAV}^{t-1}$ \\

	}
	\KwOut{  \\
	    \vspace{.42em}
	    \hspace{.5em}Drone pose: $\textbf{P}_{UAV}^{t}$\;
	    % \vspace{.23em}
        }
    \SetKwFunction{FMain}{object\_extraction}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$\mathcal{P}_{raw}^t$, $\mathcal{P}_{UAV}^{t-1}$, $\mathcal{ROI}^t_{YOLO}$}}{
        \If{$\mathcal{ROI}^t_{YOLO}$}{
            $\mathcal{P}_{roi}^t$ = $\mathcal{P}_{raw}^t$ ($\mathcal{ROI}^t_{YOLO}$)\;
        }
        \Else{
            $\mathcal{ROI}^t \longleftarrow KF \left( get\_center\left( \mathcal{P}_{UAV}^{t-1} \right) \right)$\;
            
            % $\mathcal{P}_{roi}^t$ \longleftarrow\ $\mathcal{P}^t_{raw}$ ( $\mathcal{ROI}^{t}$)\;
        }
        $\mathcal{P}^t \longleftarrow ground\_removal\left( \mathcal{P}_{ROI}^t \right)$ \;
        $\mathcal{P}_{i}^t \longleftarrow DBSCAN \left( \mathcal{P}^t \right),\:i\in(0,R)$\;
        \ForEach{ $\mathcal{P}$ $\in$ $\mathcal{P}_{i}^t$ }{%
            \If{ Min (num($\mathcal{P}$ ) - num($\mathcal{P}_{UAV}^{t-1}$) )}{%
                \If{Min (dis($\mathcal{P}$) - dis($\mathcal{P}_{UAV}^{t-1}$))}{%
                    $flag = 1$ \;
                    $\mathcal{P}^{t}_{uav} \longleftarrow \mathcal{P}$ \;
                }
                
            \Else{
                $flag = 0$\;
                }
            }
            \Else{ 
                $flag = 0$\;}
        }
    \KwRet $\mathcal{P}_{uav}^{t}$, flag \;
    }
    \ForEach{ \textit{new} $\mathcal{S}^t$ }{
        $\mathcal{ROI}^t_{YOLO} \longleftarrow\ YOLOv5 \left( \mathcal{S}^{t} \right)$\;
        \If{$\mathcal{ROI}^t_{YOLO} = \textbf{None}$}{
            $\mathcal{P}_{UAV}^{t}$ , flag = \textit{object\_extraction} ($\mathcal{P}_{raw}^t$, $\mathcal{P}_{uav}^{t-1}$) \;
            \If{flag = 0}{
                $\textbf{P}_{UAV}^{t}$ = \textit{KF\_predict} (\textit{get\_center}($\mathcal{P}_{UAV}^{t-1}$))  \;
                \textit{KF\_update} ($\textbf{P}_{UAV}^{t}$)
            }
            \Else{
                $\textbf{P}_{UAV}^{t}$ = \textit{get\_center}($\mathcal{P}_{UAV}^{t}$)  \;
                \textit{KF\_update} ($\textbf{P}_{UAV}^{t}$)  \;
            }
        }
        \Else{
            $\mathcal{P}_{UAV}^{t} = object\_extraction \left( \mathcal{P}_{raw}^t, \:\mathcal{P}_{UAV}^{t-1}, \:\mathcal{ROI}^t \right)$ \;
            $\textbf{P}_{UAV}^{t} = get\_center \left(\mathcal{P}_{UAV}^{t} \right)$\;
            $KF\_update \left( \textbf{P}_{UAV}^{t} \right)$\;
        }
    }
\end{algorithm}



==> algs/evaluation-scheme.tex <==
\begin{algorithm}[h]
% \footnotesize
\DontPrintSemicolon
\SetNoFillComment
% \SetAlgoNoLine
    \caption{The evaluation scheme}
    \label{alg:eva-scheme}
    % \centering
    \KwIn{\\
        % \vspace{.42em}
	\hspace{1em} Range image: $rng$ \\
        % \hspace{1em} Signal image: $sig$ \\
        % \hspace{1em} Point cloud: $pc$ \\
        \hspace{1em} Combinations in Table~\ref{tab:combinations}: $\textit{combs} = [\textit{comb\_i}]$, $i\in(0\sim6) $
    }
    \BlankLine
    \KwOut{\\
        \hspace{1em} Translation error: \(trans\_err\;(mean/rmse, unit:\,m)\) \\
        \hspace{1em} Rotation error: \(rot\_err\;(mean/rmse, unit:\,^\circ)\) \\
    }
    \BlankLine

    \tcc{Variable Declarations:}
$Kp$ : Keypoint \\
$pc_{kp}$: Point Cloud Keypoint \\
% \textit{en\_img}: Enhanced image \\
\textit{LOC} : LiDAR Odometry Calculation \\
\textit{GT} : Ground Truth   \\

\vspace{0.23em}
    \tcc{Image preprocess for brighter images}
    \SetKwFunction{gamma}{gamma}
    \SetKwFunction{histequal}{hist\_equalizer}
    \SetKwFunction{FPreproc}{img\_preprocess}
    % \SetKwProg{Fn}{Function}{:}{}
    \SetKwProg{Fn}{def}{:}{}
    \Fn{\FPreproc{$img$}}{
        % $img$ = {$sig$,$rng$}
        \If{$img$ == $rng$}{
            $img_{prc}$ $\gets$ \gamma($img$)\;
        }
        \Else{
            % \tcc{Keep pixels with a brightness greater than $p\_thresh$}
            \If{$pixel\_value < p\_thresh$}{     
                % \tcc{Adaptive Histogram Equalization Transform}
                $img\_hist$ $\gets$ \histequal($img$)\;     
                $img\_prc$ $\gets$ \gamma($img\_hist$)\;
                % $img\_{prc}$[$area\_w$] $\gets$ $img$[$area\_w$] \\    
                % }
                % mask = [$pixel\_value$ $\geq$ $p\_thresh$] \\
                % $area\_w$ = $img$[mask] \
            }
        }
        \KwRet $img\_{prc}$; 
        }
    \BlankLine
    \tcc{Key point detect & track}
    \SetKwFunction{MnnMatcher}{MnnMatcher}
    \SetKwFunction{FTracker}{kp\_detect\&track}
    \SetKwFunction{FColorization}{colorization}
    \SetKwFunction{FSuperresolution}{super\_resolution}
    \SetKwFunction{FKeypointdet}{keypoint\_detect}
    \SetKwProg{Fn}{def}{:}{}
    \Fn{\FTracker{\textit{img}, $kps_{t-1}$}}{
        % $pts_{t}$ $\gets$ round( $pts_{t}$ )\;
            % \tcc*[r]{Find matches using the MNN matcher in OpenCV}
            $kps_{t}$ $\gets$ \FKeypointdet(\textit{img}) \;
            $matches$ $\gets$ \MnnMatcher{$kps_{t-1}$, $kps_{t}$}\;
            mkps $\gets$ $kps_{t}$[$matches$]\;
            % mpts2 $\gets$ $kps_{t}$[$matches[:, 1]$]\;
            % N\_matches $\gets$ len(matches)\;
            % \tcc*[r]{Collect matched points coordinates}
            % current\_frame\_points $\gets$ \{(round(p2)) $\mid$ p2 $\in$ mpts2\}\;
        \KwRet{mkps}\;
    }
    \ForEach{$\textit{comb\_i}$ in $\textit{combs}$}{
    \tcc{In table\ref{tab:combinations},there are different $rng$ and $sig$ in comb}
        $rng$ = \FPreproc{$rng$}\;  
        $sig$ = \FPreproc{$sig$}\;
        \textbf{Perform} following process to every $rng$ in comb  \;
        \textit{en\_img} $\gets$ \FSuperresolution{$rng$}  \\
        % pts, desc $\gets$ \FKeypointdet(\textit{en\_img})\\
        $kp$ $\gets$ \FTracker{\textit{en\_img}, $kpts_{t-1}$}\\
        $pc_{kp}^{r}$ $\gets$ pc[index[$kp$]] \\
        \tcp*[h]{----------------------------------------------------}


        \textbf{Perform} following process to every \textbf{$sig$} in comb  \;
        
        % \If{$rng\_xt$ in \textit{comb\_i}}{
        %     $rng\_xt$ = \textit{super\_resolution($rng$)}\;
        % }
        
        % \If{$sig\_xt$ in \textit{comb\_i}}{
        %     $sig\_xt$ = \textit{super\_resolution($sig$)}\;
        %     If{ $sig\_xt_cl$ in \textit{comb\_i}}{
            
        %     }
        % }
        % \textit{img} $\gets$ \textit{Image preprocessing}($\textit{comb\_i}$) \\
        \textit{en\_img} $\gets$ \FSuperresolution{$sig$}  \\  
        \textit{en\_img} $\gets$ \FColorization{\textit{en\_img}}  \\
        % pts, desc $\gets$ \FKeypointdet\textit{en\_img})\\
        $kp$ $\gets$ \FTracker{\textit{en\_img}, $kpts_{t-1}$}\\
        $pc_{kp}^{s}$ $\gets$ pc[index[$kp$]] \\
        \tcp*[h]{----------------------------------------------------}
        $pc_{kp}$ $\gets$ integrate ($pc_{kp}^{r}$, $pc_{kp}^{s}$ )  \\
        % LO calculation with point cloud keypoint as input  \\
        Odom $\gets$ \textit{LOC}($pc_{kp}$) \\
        % Translation and rotation error computation \\
        \textit{trans\_err}, \textit{rot\_err} $\gets$ evo(Odom,GT) 
        \\
    }
\end{algorithm}

==> algs/pos_gd.tex <==


\begin{algorithm}[t]
    %
    %
    %
    \footnotesize
	\caption{\footnotesize Ground truth extraction}
	\label{alg:tracking}
	\KwIn{\\
	    \begin{tabular}{ll}
	        3D lidar point cloud:             & $\mathcal{P}$ \\
	        Last known MAV state:              & $ \textbf{p}^{k-1}_{MAV}, {\dot{\textbf{p}}_{MAV}}^{k-1}$ \\[+0.4em]
	    \end{tabular}
	}
	\KwOut{\\
	    \begin{tabular}{ll}
	        MAV state:      & \{${\textbf{p}^{k}_{MAV}}, \:\dot{\textbf{p}}^{k}_{MAV}\}$ \\[+0.2em] 
	    \end{tabular}
	}  
	%\BlankLine
	%
	\SetKwFunction{FSub}{$object\_extraction\left(\mathcal{P}, \:{\textbf{p}^{k-1}_{MAV}}, \:\dot{\textbf{p}}^{k-1}_{MAV}\right)$}
    \SetKwProg{Fn}{Function}{:}{}
    % Position estimation based on current PointCloud and last position and speed
    \BlankLine
%     \Fn{\FSub}
%     {
%             \vspace{.3em}
            
%             \KwRet ${\textbf{p}^{k}_{MAV}};$
%     }
% 	\BlankLine
    %
% 	$Adaptive\;Integrate\;Rate: I_{rate}$ \\
    % Calculate with high frequency, get the pose(high accuracy, but not robust)  
    % Coarse first, then fine grained estimate
    % \tcp{Coarse but persistent tracking}
    % \While{new $\mathcal{P}_{k}(I^{k}_{MF})$}{
    %     ${\textbf{p}^{k'}_{MAV}} =  object\_extraction(\mathcal{P}_{k}(I^{k}_{MF}), I^{k}_{MF}, \textbf{p}^{k-1}_{MAV}, \dot{\textbf{p}}^{k-1}_{MAV});$ \\
    %     % $Evaluate \; Estimation({\textbf{p}^{k-1}_{MAV}}, {\textbf{p}^{k}_{MAV}} )$ \\
    %     % $Update({\textbf{p}}^{k}, I_{rate} )$ \\
    % }
    % \tcp{Fine-grained estimation}
    \While{new $\mathcal{P}_{k}$}{
        \begin{tabular}{ll}
                Generate KD Tree:       & $kdtree \leftarrow \mathcal{P};$ \\
                MAV pos estimation:     & $\hat{\textbf{p}}_{\tiny MAV}^{k} \leftarrow \textbf{p}^{k-1}_{MAV} + \frac{\dot{\textbf{p}}_{MAV}^{k-1}}{I};$ \\[+0.4em]
                MAV points:             & $\mathcal{P}^{k}_{MAV} = KNN(kdtree, \: \hat{\textbf{p}}_{MAV}^{k});$ \\[+0.4em]
                MAV state estimation:   & ${\textbf{p}^{k}_{MAV}} = \frac{1}{\lvert\mathcal{P}^{k}_{MAV}\rvert}\sum_{p\in\mathcal{P}^{k}_{MAV}} p;$ \\
        \end{tabular}
        % ${\textbf{p}^{k''}_{MAV}} =  object\_extraction(\mathcal{P}_{k}, \textbf{p}^{k-1}_{MAV}, \dot{\textbf{p}}^{k-1}_{MAV});$ \\
        % ${\textbf{p}^{k}_{MAV}}, \: {\dot{\textbf{p}}^{k}_{MAV}} \leftarrow estimate\left(\textbf{p}^{k'}_{MAV}, \:\textbf{p}^{k''}_{MAV}\right)$\;
    }
    % $\{I^{k}_{HF}, I^{k}_{MF}\} \leftarrow adjust\_integration\_freqs\left(\textbf{p}^{k}_{MAV}, \dot{\textbf{p}}^{k}_{MAV}\right);$ \\[+0.4em]
    % $\dot{\textbf{q}}^{k}_{UGV} \leftarrow keep\_within\_FoV\left(\textbf{p}^{k}_{MAV}, \dot{\textbf{p}}^{k}_{MAV}\right);$
    
 
\end{algorithm}

==> algs/test.tex <==
\begin{algorithm}[h]
% \footnotesize
\DontPrintSemicolon
\SetNoFillComment
% \SetAlgoNoLine
    \caption{The evaluation scheme}
    \label{alg:eva-test}
    % \centering
    \KwIn{\\
        % \vspace{.42em}
	\hspace{1em} Range image: $rng$ \\
        \hspace{1em} Signal image: $sig$ \\
        \hspace{1em} Point cloud: $pc$ \\
        \hspace{1em} Combinations in Table~\ref{tab:combinations}: $\textit{combs} = [\textit{comb\_i}]$, $i\in(0\sim6) $
    }
    \BlankLine
    \KwOut{\\
        \hspace{1em} Translation error: \(trans\_err\;(mean/rmse, unit:\,m)\) \\
        \hspace{1em} Rotation error: \(rot\_err\;(mean/rmse, unit:\,^\circ)\) \\
    }
    \BlankLine

    \tcc{Variable Declarations:}
$kps_{t}$ : Current Key points \;
$mkpts_{t}$ : matched Key points\;
$pc_{kp}$: Point cloud corresponded to key points \;
% \textit{en\_img}: Enhanced image \\
\textit{LOC} : LiDAR odometry calculation \;
\textit{GT} : Ground truth  \;
\BlankLine
    \tcc{Image preprocess for brighter images}
    \SetKwFunction{gamma}{gamma}
    \SetKwFunction{histequal}{hist\_equalizer}
    \SetKwFunction{FPreproc}{img\_preprocess}
    % \SetKwProg{Fn}{Function}{:}{}
    \SetKwProg{Fn}{def}{:}{}
    \Fn{\FPreproc{$img$}}{
        % $img$ = {$sig$,$rng$}
        \If{$img$ == $rng$}{
            $img_{prc}$ $\gets$ \gamma($img$)\;
        }
        \Else{
            % \tcc{Keep pixels with a brightness greater than $p\_thresh$}
            \If{$pixel\_value < p\_thresh$}{     
                % \tcc{Adaptive Histogram Equalization Transform}
                $img\_hist$ $\gets$ \histequal($img$)\;     
                $img\_prc$ $\gets$ \gamma($img\_hist$)\;
                % $img\_{prc}$[$area\_w$] $\gets$ $img$[$area\_w$] \\    
                % }
                % mask = [$pixel\_value$ $\geq$ $p\_thresh$] \\
                % $area\_w$ = $img$[mask] \
            }
        }
        \KwRet $img\_{prc}$; 
        }
    \BlankLine
    \tcc{Key point detect \& track}
    \SetKwFunction{FLOC}{LOC}
    \SetKwFunction{FEVO}{EVO}
    \SetKwFunction{FCombine}{Combine}
    \SetKwFunction{MnnMatcher}{MnnMatcher}
    \SetKwFunction{FTracker}{kp\_tracker}
    \SetKwFunction{FColorization}{colorization}
    \SetKwFunction{FSuperresolution}{super\_resolution}
    \SetKwFunction{FKeypointdet}{keypoint\_detect}
    \SetKwProg{Fn}{def}{:}{}
    \Fn{\FTracker{$kps_{t}$, $kps_{t-1}$}}{
        % $pts_{t}$ $\gets$ round( $pts_{t}$ )\;
            % \tcc*[r]{Find matches using the MNN matcher in OpenCV}
            $matches$ $\gets$ \MnnMatcher{$kps_{t-1}$, $kps_{t}$}\;
            mkps $\gets$ $kps_{t}$[$matches$]\;
            % mpts2 $\gets$ $kps_{t}$[$matches[:, 1]$]\;
            % N\_matches $\gets$ len(matches)\;
            % \tcc*[r]{Collect matched points coordinates}
            % current\_frame\_points $\gets$ \{(round(p2)) $\mid$ p2 $\in$ mpts2\}\;
        \KwRet{mkps}\;
    }
    % \ForEach{$\textit{comb\_i}$ in $\textit{combs}$}{
         
        
        % \textbf{Perform} following process to every $rng$ in comb  \;
    $rng$ = \FPreproc{$rng$}\; 
    \textit{$rng_{2r}$} $\gets$ \FSuperresolution{$rng$}  \\
    % $kp$ $\gets$ \FTracker{\textit{en\_img}, $kpts_{t-1}$}\\
    % $pc_{kp}^{r}$ $\gets$ pc[index[$kp$]] \\
    % \tcp*[h]{----------------------------------------------------}
    % \textbf{Perform} following process to every \textbf{$sig$} in comb  \;
    $sig$ = \FPreproc{$sig$}\;
    $sig^{c}$ $\gets$ \FColorization{$sig$}  \\
    $sig_{2r}$ $\gets$ \FSuperresolution{$sig$}  \\  
    $sig_{2r}^{c}$ $\gets$ \FColorization{$sig_{2r}$}  \\
    % \tcp*[h]{----------------------------------------------------}
    \tcc{Arrange and combine $sig$, $rng$, $rng_{2r}$, $sig_{2r}$,$sig_{2r}^{c}$,$sig^{c}$ to be \textit{comb} in table~\ref{tab:combinations}}
    \ForEach{$\textit{comb\_i}$ in $combs$}{
        % pts, desc $\gets$ \FKeypointdet\textit{en\_img})\\
        \ForEach{$\textit{img}$ in $\textit{comb\_i} $}{

        $kps_{t}$ $\gets$ \FKeypointdet(\textit{img}) \;
        $mkpts_{t}$ $\gets$ \FTracker{$kps_{t}$, $kps_{t-1}$}\\
        $pc_{kp}^{i}$ $\gets$ pc[index[$mkpts_{t}$]] \\
}
        $pc_{kp}$ $\gets$ \FCombine{$pc_{kp}^{i}$} \\
        % LO calculation with point cloud keypoint as input  \\
        $Odom$ $\gets$ \FLOC{$pc_{kp}$} \\
        % Translation and rotation error computation \\
        \textit{trans\_err}, \textit{rot\_err} $\gets$ \FEVO{$Odom$,GT} 
        \\
    }
\end{algorithm}

==> sec/00_Abstract.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%%                ABSTRACT                  %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\IEEEtitleabstractindextext{%
\fcolorbox{abstractbg}{abstractbg}{%
\begin{minipage}{\textwidth}%
% \begin{wrapfigure}[13]{r}{0.42\textwidth}%
% \includegraphics[width=0.4\textwidth]{fig/abstract-img.png}%
% \end{wrapfigure}%
\begin{abstract}%
    \label{sec:abstract}%
    In recent years, Light Detection and Ranging (LiDAR) technology, a critical sensor in robotics and autonomous systems, has seen significant advancements. These improvements include enhanced resolution of point clouds and the capability to provide 360\textdegree\, low-resolution images. These images encode various data such as depth, reflectivity, and near-infrared light within the pixels. However, an excessive density of points and conventional point cloud sampling can be counterproductive, particularly in applications such as LiDAR odometry, where misleading points and degraded geometry information may induce drift errors.  Currently, extensive research efforts are being directed towards leveraging LiDAR-generated images to improve situational awareness. 
    
    This paper presents a comprehensive review of current deep learning (DL) techniques, including colorization and super-resolution, which are traditionally utilized in conventional computer vision tasks. These techniques are applied to LiDAR-generated images and are analyzed qualitatively. Based on this analysis, we have developed a novel approach that selectively integrates the most suited colorization and super-resolution methods with LiDAR imagery to sample reliable points from the LiDAR point cloud. This approach aims to not only improve the accuracy of point cloud registration but also avoid mismatching caused by lacking geometry information, thereby augmenting the utility and precision of LiDAR systems in practical applications. In our evaluation, the proposed approach demonstrates superior performance compared to our previous work, achieving lower translation and rotation errors with a reduced number of points.
\end{abstract}

\begin{IEEEkeywords}
    LiDAR, Odometry, Super-Resolution, Colorization,  LiDAR-as-a-camera, Point Cloud Sampling
\end{IEEEkeywords}
\end{minipage}}}

==> tbs/result-error.tex <==
\begin{table*}[t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llcclll@{}}
\toprule
\multicolumn{2}{c}{\textbf{Combination}} & \textbf{Open road}                     & \textbf{Forest}                         & \textbf{Lab space (hard)}             & \textbf{Lab space (easy)}       & \textbf{Hall (large)}                  \\ 

\multicolumn{7}{c}{(Translation error (mean/rmse), rotation error (mean))} \\

\midrule

\multicolumn{2}{c}{comb\_0}  & (1.055/1.222, 1.782) & (0.086/0.102, 1.666) & (0.094/0.107, 1.185) & (0.083/0.095, 1.143) & (0.457/0.500, \textbf{0.903}) \\

\multicolumn{2}{c}{comb\_1}  & (0.605/0.731, 1.855) & (0.087/0.103, 1.663) & (0.120/0.136, 1.398) & (0.098/0.115, 1.216) & (0.485/0.532, 0.955) \\

\multicolumn{2}{c}{comb\_2} & (\textbf{0.357/0.409}, 1.808)  & (0.087/0.102, 1.668) & (0.126/0.149, 1.473) & (0.097/0.110, 1.186) & (0.456/0.500, 0.903) \\

\multicolumn{2}{c}{comb\_3} & (5.726/6.738, 1.957)  & (0.086/\textbf{0.102}, 1.666) & (0.045/0.050, \textbf{0.721}) & (0.032/0.036, \textbf{0.657}) & (\textbf{0.438/0.476}, 0.920) \\

\multicolumn{2}{c}{comb\_4} & (1.464/1.641, 1.806)  & (0.086/0.102, \textbf{1.662}) & (0.092/0.104, 1.235) & (0.080/0.095, 1.066) &    (1.175/1.326, 0.929) \\

\multicolumn{2}{c}{comb\_5} & (1.052/1.307, 1.807)  & (0.088/0.103, 1.672) & (0.101/0.114, 1.213) & (0.089/0.105, 1.118) &    (0.456/0.503, 0.922) \\ 

\multicolumn{2}{c}{comb\_6} & (0.492/0.595, 1.806)  & (0.086/0.103, 1.668) & (0.109/0.123, 1.319) & (0.093/0.107, 1.156) &    (0.452/0.498, 0.929) \\ 

\midrule

\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Prior work~\cite{zhang2023lidar}\\ (\textit{rng\_sig)}\end{tabular}} &4\_7  & (0.817/0.952, 2.33) & (0.082/0.102, 7.88) & (0.039/0.046, 1.46) & (0.027/0.033, 0.98) & (0.583/0.660, 2.88) \\

&5\_5  & (2.176/2.410, \textbf{1.76}) & (0.108/0.203, 6.96) & (0.037/\textbf{0.043}, 1.35) & (0.027/0.032, 0.97) & (0.707/0.801, 2.66) \\

&7\_5  & (1.784/2.006, 2.30)  & \textbf{0.080}/0.102, 7.22) & (\textbf{0.033}/0.047, 1.59) & (\textbf{0.025/0.028}, 0.97) & (0.698/0.803, 3.11)  \\ \bottomrule
\end{tabular}
}
\caption{Comparison of translation and rotation errors across various combinations of DL-based super-resolution and colorization methods shown in Table~\ref{tab:combinations}, benchmarked against the results reported in prior work~\cite{zhang2023lidar}. In the table, 
\textit{sig} and \textit{rng} represent the size of neighboring point areas for the signal and range images, respectively, denoted as \textit{sig\_rng}.
}
\label{tab:error}
\end{table*}

==> tbs/result-points.tex <==
\begin{table}[]
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}llccccc@{}}
\toprule
\multicolumn{2}{c}{\textbf{Combination}} & \textbf{Open road} & \textbf{Forest} & \textbf{Lab space (hard)} & \textbf{Lab space (easy)} & \textbf{Hall (large)} \\ 

\multicolumn{7}{c}{(Number of Points (pts))} \\

\midrule

\multicolumn{2}{c}{comb\_0}     & 1149      & 1131   & 1613             & 1589             & 1492         \\
\multicolumn{2}{c}{comb\_1}     & 628       & 826    & 999              & 970              & 875          \\
\multicolumn{2}{c}{comb\_2}     & 787       & 820    & 1264             & 1229             & 1093         \\
\multicolumn{2}{c}{comb\_3}     & 1310      & 1167   & 1796             & 1270             & 1731         \\
\multicolumn{2}{c}{comb\_4}     & 1317      & 1170   & 2053             & 2031             & 1737         \\
\multicolumn{2}{c}{comb\_5}     & 1028      & 732    & 1587             & 1571             & 1322         \\ 
\multicolumn{2}{c}{comb\_6}     & 793       & 823    & 1396             & 1370             & 1099         \\ 

\midrule

\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Prior work~\cite{zhang2023lidar}\\ (\textit{rng\_sig)}\end{tabular}} 

&4\_7          & 4784 & 11447  & 9518             & 9392            & 7094          \\

&5\_5          & 3183 & 7568   & 6446             & 6292            & 4783          \\

&7\_5          & 4756 & 11627  & 9469             & 9378            & 7078          \\ \bottomrule
\end{tabular}
}
\caption{Comparison of the number of points across various combinations of DL-based super-resolution and colorization methods shown in Table~\ref{tab:combinations}, benchmarked against the results reported in prior work~\cite{zhang2023lidar}.In the table, 
\textit{sig} and \textit{rng} represent the size of neighboring point areas for the signal and range images, respectively, denoted as \textit{sig\_rng}.}
\label{tab:points}
\end{table}

==> tex/XYZ_plot/XY_plot_seq3.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{1,0.188235294117647,0.188235294117647}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(1.35,1.00)},
  anchor=south east,
  draw=white,
  /tikz/every even column/.append style={column sep=0.5cm},
},
legend columns=3,
axis line style= {white},
tick align=outside,
tick pos=left,
% title={XY plot},
xmajorgrids,
xmajorticks=true,
xminorgrids,
xminorgrids=true,
ymajorgrids,
ymajorticks=true,
yminorgrids,
yminorgrids=true,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
        minor tick num = 3,
        minor grid style={dashed},
x grid style={white!69.0196078431373!black},
xmin=2.2937600641077, xmax=4.02480477083426,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=2.12877276002231, ymax=5.16023554096054,
ytick style={color=black}
]
\addplot [line width=1pt, color1]
table {%
2.73259080042564 2.2954216427211
2.74343163560815 2.31777733333452
2.76226672899973 2.33763132237825
2.77197038543539 2.37099891932597
2.77941772327846 2.39915270681096
2.78829972509503 2.43237971210357
2.79987289003186 2.48228843678183
2.81119314984344 2.50723591521166
2.80290796777034 2.57016757457341
2.79863298401608 2.61110224606921
2.77857855552648 2.65472841443386
2.76879705733064 2.69645540690029
2.75941210404591 2.73302168382298
2.73673221300456 2.78460398196515
2.72048243208293 2.83162000452564
2.70981135271734 2.87356750945619
2.70740219155114 2.92110874032325
2.72064163397116 2.97777074365821
2.74227311431043 3.02254324868717
2.76767565170557 3.09168373521269
2.79776355687598 3.13921476015578
2.84619489817872 3.20421169494298
2.87781080242177 3.26403626073103
2.91866555366626 3.308839878853
2.95885920391216 3.35316934072594
2.99111507738432 3.39633428969372
3.01853055180776 3.43829247711476
3.04301459264569 3.47959461117091
3.07663927060839 3.50625344126635
3.11054872763804 3.52119343091084
3.12983829173943 3.55705093628962
3.17180958828291 3.58359333367066
3.22576927251157 3.61456898100191
3.28173252084285 3.66382379414986
3.33522348003846 3.70350267599603
3.38826456094178 3.73986772656383
3.42938132912533 3.79459211832735
3.47478516109619 3.8589167167674
3.49920348070984 3.92124063459251
3.51926711555732 3.99992257838136
3.53323378630256 4.04932519277265
3.5104876649043 4.12635767857896
3.50924029339517 4.18267360064715
3.49381577645071 4.26760867678425
3.46585263690297 4.33154077984819
3.42616129615141 4.40008314812554
3.39381158144173 4.44440381051309
3.35878389826143 4.50073852441353
3.31842252627628 4.54387388862518
3.28373377124474 4.57784565316582
3.26717255524395 4.61861403199193
3.20625048331003 4.65154330276112
3.14292769800767 4.64713122150596
3.10984578909261 4.65879743126192
3.03028290664255 4.70050728512957
2.98342308024528 4.71491058954871
2.90833750529192 4.66791998111957
2.81369016358825 4.66456338564272
2.68960518051834 4.6514615485341
2.61834317180246 4.61419404518564
2.59133359628131 4.57197420706711
2.53889867078703 4.53758470508788
2.49640102134837 4.46912709671841
2.43093337475764 4.42916135383894
2.41406072727463 4.34431157821041
2.38916320019083 4.25510880352394
2.38424727687088 4.19943957942588
2.3797065920442 4.10868519659685
2.3804940506239 4.03084815122655
2.38711249426717 3.96403028690104
2.38454997523936 3.87862436703802
2.38524487352131 3.81631763394191
2.4086064252633 3.75911789075354
2.44214202121798 3.71140899378346
2.47419208213707 3.65434881455194
2.52827375525438 3.60680009805964
2.59370041123844 3.58652056216466
2.64731952288101 3.55043822523879
2.73361202424747 3.53340288012352
2.81427216858312 3.52469800454746
2.90816328526587 3.52613146215501
2.96942244815454 3.50699401464921
3.04041606903737 3.54187917205913
3.08431936930925 3.53992240245697
3.13378486714116 3.55999978636447
3.15156481646775 3.58142860940515
3.19113576408744 3.59744380239372
3.20853207243552 3.61509018467778
3.22592080248474 3.64513837855198
3.24157625200172 3.67737153279367
3.26849122905683 3.70888977791336
3.29794225893743 3.76111119411413
3.34512934296052 3.81567450582051
3.3871017149695 3.87873492581653
3.44399595481758 3.94845073923546
3.50091762439694 4.00428374323119
3.55147346702835 4.07382113314224
3.58816732015563 4.13568268890664
3.61049923891057 4.22094809638009
3.60773687233267 4.28045051725409
3.60600726786476 4.35828816630771
3.55194239633667 4.4285547032453
3.51784149259861 4.47791919068106
3.43165381383551 4.55688852191186
3.36386457197198 4.62122417091992
3.29561769526148 4.68121848605205
3.24881431706591 4.73146398329164
3.20861244380214 4.78350441257105
3.16938767019224 4.83617557570634
3.18050056208889 4.88170283359478
3.16503509773993 4.93427000544225
3.208614253057 4.95618168663791
3.18412356131201 4.95904613541331
3.21190362926877 4.97156268814394
3.21027400805481 4.96111937046137
3.1700639722792 4.95360187519411
3.11517225580331 4.94110527615339
3.07335484285838 4.90874431955096
2.99570056124122 4.88445928190409
2.85846299112991 4.84402526283237
2.78757485262802 4.81363791051145
2.74221472731354 4.74639621909141
2.63435390947082 4.70270904061743
2.56660606991018 4.64008299046569
2.51794481030488 4.57376563144212
2.46911614289648 4.49753014236375
2.45058709697382 4.4323391667904
2.47135825381675 4.3752508721595
2.45283485458011 4.30350269834918
2.49496367430251 4.23780888271187
2.48904701255822 4.16120874459902
2.5646343025954 4.08395576213948
2.5687428966418 3.99330635987506
2.58730541323742 3.90717893497241
2.62251700243816 3.82396238528935
2.64333416476756 3.73051040945206
2.67948897550178 3.67380135412162
2.72166591565624 3.62732310185697
2.75270055594358 3.60816445200711
2.80677818151326 3.6098946166593
2.85133018420882 3.62974614417943
2.91066751505617 3.63564250016771
2.98482763034345 3.67777015015346
3.06730554673034 3.71591579123588
3.14460274091814 3.75898147583426
3.23213784635088 3.79552346889038
3.31024163079453 3.82217176546725
3.3512951091394 3.85307696350958
3.4017711046021 3.88682844445628
3.38549056476237 3.88813003946867
3.40526244113241 3.89499281734444
3.40346612365705 3.89927045065691
3.39371821855194 3.86211921707423
3.4019140630963 3.8675035459905
3.43280327400255 3.8550389843343
3.42039131920034 3.84582553031054
3.47478814252454 3.82192860675603
3.52481279222092 3.8188104365502
3.59465430557435 3.81326090765918
3.64292121266644 3.79713954466694
3.71732876891936 3.77813464376112
3.78228755694404 3.76760799931913
3.84326397997338 3.73444576200688
3.87591104971136 3.70009956408722
3.90045321168651 3.64725299707619
3.91996780654539 3.57459200766659
3.89384541236475 3.49507137704457
3.8532622045896 3.40462543050264
3.8009317601632 3.31878053771735
3.747730859615 3.21306244747252
3.66707106515983 3.11988218513941
3.5915272141181 3.03607055697764
3.52093959907854 2.95875103539358
3.45350962038186 2.90943214434925
};
\addlegendentry{Ours }
\addplot [line width=1pt, color0]
table {%
2.73138986085617 2.26656652279223
2.75360432320259 2.35714382130048
2.7508083515257 2.46912835587662
2.74550851348316 2.54904439484317
2.72250258307611 2.61610617873149
2.70890036336189 2.67091839597072
2.70048674867281 2.71293841304514
2.6621245905157 2.8289300166783
2.65258940451437 2.8774984141375
2.65388347721636 2.9297412196155
2.67367372667819 2.99582687673874
2.71430448120537 3.04398971125765
2.75246716597602 3.11821334733149
2.86294371432932 3.23500900778058
2.90622962533318 3.29710121648793
2.95056109235385 3.34523716767429
2.99364341688218 3.38133012793502
3.02859427991752 3.42218117361351
3.05303250126545 3.46468232077013
3.07371619488321 3.50232048035524
3.13888316455779 3.53138675226301
3.16026821946876 3.56050365837881
3.2011036391208 3.5866636872793
3.26194031975455 3.61679437274807
3.324686196072 3.66508438167831
3.39168199789358 3.71110243709038
3.45507064740115 3.74881729731915
3.54791406710348 3.87321212722207
3.56893738355065 3.94332451694098
3.57555290050113 4.02933308877975
3.58155283205009 4.09019776487595
3.54932629113885 4.16508434190537
3.53567629037423 4.22440220256894
3.51997284555271 4.30491172300629
3.433437696447 4.45110679138145
3.39377508547388 4.49818151091311
3.35114383424233 4.54490620065661
3.31313908978661 4.58474715181891
3.28820382358359 4.61732776598191
3.27425116100906 4.64513056496436
3.21557335445532 4.68209119320882
3.09517642619145 4.67689255581475
3.0237912725378 4.71121890184527
2.96730721438741 4.72908747193449
2.88654480121457 4.68988240652772
2.7825827012005 4.67061365107596
2.66926498137833 4.66318354414061
2.56055966975768 4.62011394913901
2.49794002158032 4.52897023159987
2.46771011458673 4.45192419369431
2.41016471761844 4.40100904910164
2.38746546621496 4.31615609623814
2.38373945569784 4.22276895453488
2.37568340169178 4.1513383273049
2.37438529736967 4.06132088987714
2.39164826922535 3.91240201883462
2.3902769834158 3.83365064700832
2.38948524431167 3.76827987219866
2.40738441948655 3.71381407610171
2.45310103488526 3.67536896327288
2.49340311007651 3.62523566406642
2.55163154853127 3.57816940186485
2.69675335918421 3.53342552792813
2.7828881224921 3.51982087848909
2.8781491291644 3.51785614866331
2.97401096266729 3.52830366103386
3.04490491628471 3.51297702842778
3.10674838697937 3.54607893560372
3.14268939458707 3.56705205771726
3.19304735985892 3.60401281076548
3.21979241206349 3.62928634441175
3.23261212494025 3.64446115856433
3.24157911978149 3.67286715948425
3.25282331608796 3.71002245775272
3.27531500357294 3.74868867147703
3.30946525165874 3.80102292687833
3.42385911017909 3.93236281040655
3.4925721935755 4.00647533265346
3.55868134397623 4.06658877149959
3.62211398508616 4.13244637976297
3.65590555658562 4.1961475001081
3.66762449416404 4.27739257805573
3.65635034189895 4.34797240131824
3.57450225759951 4.49815402389132
3.5158561928853 4.55318674767089
3.41539104845262 4.63109920128498
3.33620951102076 4.70003778680557
3.25981144745224 4.76173411000382
3.21774691837508 4.80983644276065
3.18190880196593 4.85795678179988
3.17415752571927 4.94957756098052
3.17693561005654 5.00200282074395
3.22823553566057 5.02244177819062
3.23357894433589 5.01361867542625
3.25220577008086 5.01083580216477
3.2515280013004 4.99080038985157
3.20585824063552 4.97426244268442
3.06770239653192 4.92098387821703
2.97668730023826 4.89068955830255
2.84576909514051 4.85105684806315
2.72324522445048 4.81949275852938
2.66511587162346 4.75215494766644
2.56737987444208 4.7000965492915
2.49471329396189 4.6370482848981
2.4093239167304 4.48600491487912
2.39956970376416 4.4143954307876
2.4376903406125 4.35508778149186
2.44608059076592 4.28856147136882
2.49113634814668 4.21924292669192
2.49765126578515 4.14232480811796
2.57138202453032 4.05807420954335
2.60142040165522 3.87004989365037
2.63148326539495 3.78420504498652
2.65489646110252 3.69286429381683
2.67590307732644 3.63283440896259
2.71555056669599 3.60052766507381
2.75553028398983 3.59385470673663
2.80934333571462 3.61573660602321
2.92733741621492 3.67854550142618
3.00795400936487 3.72883539212453
3.113924435822 3.78066445016795
3.20209421874616 3.82685738124627
3.29513009591462 3.86869615050429
3.37406738163484 3.89120954533684
3.41678144100867 3.91382799082125
3.42748138373125 3.9365317018496
3.41629296783595 3.93210645408647
3.39991136029194 3.93231502623131
3.38655207560852 3.89157036167549
3.38100526590359 3.87612959104443
3.41160372311744 3.86039258272765
3.42411932536854 3.84920205010396
3.46911867279182 3.82223804415004
3.62774585499471 3.81118702895529
3.68700583597362 3.78918835850452
3.76279959859637 3.76273740012428
3.83677982126538 3.74379930250183
3.89950867841041 3.71244778006224
3.93350333458381 3.66098633321622
3.94612092052851 3.51781356500873
3.90038448028181 3.42482929034603
3.83280522309102 3.32435618429358
3.75225049030137 3.22850809599341
3.67462506650057 3.12001769870334
3.57868141193329 3.02508054511676
3.48884590654207 2.9409249519996
3.33868769525814 2.83436894351627
3.27961156151381 2.79343853460443
3.24219519876619 2.76691028471854
};
\addlegendentry{Point Cloud}
% \addplot [line width=1pt, green!50!black]
% table {%
% 2.79194092027163 2.35892892452518
% 2.79407119406988 2.42978630582589
% 2.79527527534208 2.48453329989567
% 2.79418461279521 2.53544276599431
% 2.7992917117979 2.60163917930246
% 2.81102871558341 2.63961579753378
% 2.79760860772589 2.70738974953776
% 2.78645569767935 2.75855673276656
% 2.75987040227934 2.8035775783111
% 2.74492820427677 2.84376380208128
% 2.73700166567946 2.8750528381069
% 2.71236227704775 2.92158934911775
% 2.68765841775157 2.97520109740467
% 2.67290493528827 3.02040086164092
% 2.66640708423765 3.06965739993503
% 2.67907644603627 3.13503458401981
% 2.71122620765581 3.1852448045617
% 2.73898108045827 3.26139294599305
% 2.78053817349636 3.31810043051243
% 2.83576546128013 3.38685611116533
% 2.86746986064176 3.45422213542551
% 2.90443960573929 3.50698442114095
% };
% \addlegendentry{Image}
\addplot [line width=1pt, black, dashed]
table {%
2.78004336357117 2.44961881637573
2.78473997116089 2.49184632301331
2.78169870376587 2.53642201423645
2.77279257774353 2.5811128616333
2.7611358165741 2.62548923492432
2.74732780456543 2.66858124732971
2.73093748092651 2.71244502067566
2.69390487670898 2.80324053764343
2.68285369873047 2.84974360466003
2.68129086494446 2.89853239059448
2.68994092941284 2.95167922973633
2.7073175907135 3.00733399391174
2.73254680633545 3.06419110298157
2.80578780174255 3.17853021621704
2.84787058830261 3.23518180847168
2.89023494720459 3.28984522819519
2.9271776676178 3.34109807014465
2.96092367172241 3.38540554046631
2.99176788330078 3.42358613014221
3.02260088920593 3.4562566280365
3.08351445198059 3.50875163078308
3.11538076400757 3.53420877456665
3.15450525283813 3.55867266654968
3.20232772827148 3.58785653114319
3.25803208351135 3.6181046962738
3.3161768913269 3.65492224693298
3.37219643592834 3.70083785057068
3.47152757644653 3.80997467041016
3.50878357887268 3.87289643287659
3.53404450416565 3.93877172470093
3.54474639892578 4.00425100326538
3.54177737236023 4.07564973831177
3.5278651714325 4.14390993118286
3.50693893432617 4.21157598495483
3.44325828552246 4.34743690490723
3.41175317764282 4.3992977142334
3.38133764266968 4.44696283340454
3.34080910682678 4.50991916656494
3.31128025054932 4.55272197723389
3.27819752693176 4.59152603149414
3.23718738555908 4.62049102783203
3.13333964347839 4.66143894195557
3.0713849067688 4.67684459686279
3.00010514259338 4.68613862991333
2.93614459037781 4.68156385421753
2.84673571586609 4.67292547225952
2.7660768032074 4.65167999267578
2.68826532363892 4.62711381912231
2.56908178329468 4.56195640563965
2.4967725276947 4.48921155929565
2.45544767379761 4.42907476425171
2.42531800270081 4.364417552948
2.39972305297852 4.28832912445068
2.38822770118713 4.21258687973022
2.38112616539001 4.13534498214722
2.37244391441345 3.9815731048584
2.37436366081238 3.91040086746216
2.38197445869446 3.84459114074707
2.38410639762878 3.83271741867065
2.38410639762878 3.83271741867065
2.54188394546509 3.59143424034119
2.54188394546509 3.59143424034119
2.63489747047424 3.55322051048279
2.71523118019104 3.53378105163574
2.79587984085083 3.52052617073059
2.87371587753296 3.51484632492065
2.94537568092346 3.51649236679077
3.00989937782288 3.52600789070129
3.02894711494446 3.53686928749084
3.1410870552063 3.56351637840271
3.16888523101807 3.57629799842834
3.19266724586487 3.59665036201477
3.21331095695496 3.62381148338318
3.23522543907166 3.65565609931946
3.25612902641296 3.696049451828
3.28694272041321 3.73732781410217
3.37403917312622 3.84776592254639
3.43747353553772 3.91309595108032
3.46730494499207 3.94392347335815
3.54685282707214 4.03354120254517
3.56150364875793 4.05302429199219
3.56150364875793 4.05302429199219
3.55420994758606 4.41191577911377
3.55420994758606 4.41191577911377
3.52897119522095 4.44498062133789
3.46123027801514 4.51591968536377
3.44793391227722 4.52946996688843
3.44793391227722 4.52946996688843
3.20479941368103 4.8422794342041
3.20479941368103 4.8422794342041
3.20333743095398 4.84621095657349
3.19610905647278 4.88337802886963
3.20433259010315 4.92765474319458
3.20877623558044 4.93645238876343
3.20877623558044 4.93645238876343
3.10875654220581 4.93231248855591
3.10875654220581 4.93231248855591
3.09200954437256 4.92480373382568
3.0337131023407 4.9000825881958
2.81984186172485 4.80996656417847
2.81984186172485 4.80996656417847
2.74672770500183 4.77510261535645
2.66049242019653 4.72225284576416
2.59113669395447 4.67178773880005
2.47602367401123 4.53933477401733
2.44892525672913 4.4741735458374
2.44124889373779 4.4066367149353
2.44737863540649 4.33526086807251
2.46477293968201 4.2646312713623
2.48559141159058 4.19270467758179
2.5109715461731 4.11613798141479
2.56022667884827 3.95782518386841
2.59123277664185 3.86118698120117
2.61795139312744 3.78020834922791
2.64434695243835 3.71509742736816
2.67542433738708 3.66681861877441
2.7141900062561 3.63695573806763
2.75917601585388 3.62501287460327
2.87690043449402 3.65587210655212
2.94824028015137 3.68864607810974
3.02909922599792 3.72396874427795
3.1125910282135 3.75977635383606
3.19374990463257 3.79366683959961
3.25704741477966 3.82296109199524
3.32147431373596 3.85447812080383
3.3886239528656 3.89113712310791
3.3969361782074 3.89532256126404
3.39630007743835 3.89313435554504
3.3953697681427 3.88669848442078
3.39798903465271 3.8734872341156
3.4073429107666 3.85793447494507
3.42936635017395 3.84170961380005
3.45953583717346 3.82747554779053
3.5581591129303 3.80352425575256
3.62155294418335 3.7911856174469
3.69111347198486 3.77538084983826
3.76070165634155 3.75537896156311
3.82333898544312 3.72709131240845
3.86648988723755 3.69070506095886
3.91346454620361 3.56822967529297
3.89978837966919 3.49198365211487
3.86199855804443 3.40586566925049
3.81219482421875 3.32272267341614
3.81219482421875 3.32272267341614
3.81219482421875 3.32272267341614
3.81219482421875 3.32272267341614
3.81219482421875 3.32272267341614
3.81219482421875 3.32272267341614
3.81219482421875 3.32272267341614
};
\addlegendentry{GT}
\end{axis}

\end{tikzpicture}


==> tex/XYZ_plot/XZ_plot_seq3.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{1,0.188235294117647,0.188235294117647}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=white!80!black
},
axis line style= {white},
tick align=outside,
tick pos=left,
% title={XY plot},
xmajorgrids,
xmajorticks=true,
xminorgrids,
xminorgrids=true,
ymajorgrids,
ymajorticks=true,
yminorgrids,
yminorgrids=true,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
            minor tick num = 3,
        minor grid style={dashed},
x grid style={white!69.0196078431373!black},
xmin=2.2937600641077, xmax=4.02480477083426,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.404950771684837, ymax=1.54912152663555,
ytick style={color=black}
]
\addplot [line width=1pt, color1]
table {%
2.73259080042564 0.456958533273505
2.74343163560815 0.49487950715315
2.76226672899973 0.529290846679961
2.77197038543539 0.558159603164172
2.77941772327846 0.581603031021609
2.78829972509503 0.611786834903712
2.79987289003186 0.619828840130322
2.81119314984344 0.618996725006725
2.80290796777034 0.628498933188615
2.79863298401608 0.618617386776924
2.77857855552648 0.614607834975727
2.76879705733064 0.595761471537237
2.75941210404591 0.587547656728352
2.73673221300456 0.590958649413665
2.72048243208293 0.591881436489796
2.70981135271734 0.587976674053637
2.70740219155114 0.602002696201986
2.72064163397116 0.60076945794349
2.74227311431043 0.599485724584289
2.76767565170557 0.606668274298737
2.79776355687598 0.601798888398763
2.84619489817872 0.601803934405946
2.87781080242177 0.624994661038883
2.91866555366626 0.618054264314445
2.95885920391216 0.633184133508421
2.99111507738432 0.621581680741958
3.01853055180776 0.608653774943656
3.04301459264569 0.575099462250055
3.07663927060839 0.572568446543079
3.11054872763804 0.572684579097422
3.12983829173943 0.582454008587114
3.17180958828291 0.572830630436128
3.22576927251157 0.57180452551432
3.28173252084285 0.591655611703931
3.33522348003846 0.601012115979793
3.38826456094178 0.597981792655272
3.42938132912533 0.583684884156747
3.47478516109619 0.588966843957799
3.49920348070984 0.59836364931814
3.51926711555732 0.597582087944079
3.53323378630256 0.593434769797821
3.5104876649043 0.595421832362148
3.50924029339517 0.587168678823642
3.49381577645071 0.61323269863585
3.46585263690297 0.619632582003686
3.42616129615141 0.616422580950774
3.39381158144173 0.642036095741194
3.35878389826143 0.627756915178666
3.31842252627628 0.600471148141839
3.28373377124474 0.616949772980762
3.26717255524395 0.638238638834733
3.20625048331003 0.644806702267674
3.14292769800767 0.63367921735363
3.10984578909261 0.669634341593406
3.03028290664255 0.689264916110825
2.98342308024528 0.670265382912131
2.90833750529192 0.673432023045431
2.81369016358825 0.663546258504555
2.68960518051834 0.673433980979231
2.61834317180246 0.658970398827948
2.59133359628131 0.666703837043153
2.53889867078703 0.671934417412527
2.49640102134837 0.653844414067499
2.43093337475764 0.65968524912859
2.41406072727463 0.685358084016413
2.38916320019083 0.69307586205989
2.38424727687088 0.701937000010989
2.3797065920442 0.720095622449483
2.3804940506239 0.724435974931953
2.38711249426717 0.731778433289824
2.38454997523936 0.741309372872078
2.38524487352131 0.734836655091209
2.4086064252633 0.761445802916635
2.44214202121798 0.759670298112906
2.47419208213707 0.789383693822738
2.52827375525438 0.803059543989636
2.59370041123844 0.813322396882952
2.64731952288101 0.824897819019936
2.73361202424747 0.840585453207842
2.81427216858312 0.849309565324545
2.90816328526587 0.879255694390182
2.96942244815454 0.87885509882795
3.04041606903737 0.904607260521757
3.08431936930925 0.911776331357928
3.13378486714116 0.926187070720048
3.15156481646775 0.934689504021621
3.19113576408744 0.933546064274718
3.20853207243552 0.954467023878263
3.22592080248474 0.966678058414332
3.24157625200172 0.956835685894477
3.26849122905683 0.973457766206282
3.29794225893743 0.976457955699481
3.34512934296052 0.978880187295118
3.3871017149695 0.978734109121055
3.44399595481758 0.96995812975022
3.50091762439694 0.97968247290656
3.55147346702835 0.964835905435578
3.58816732015563 0.963451033157929
3.61049923891057 0.995157931634678
3.60773687233267 0.972477292621147
3.60600726786476 0.951715788645927
3.55194239633667 0.95058415575198
3.51784149259861 0.960707664166411
3.43165381383551 0.984419651304546
3.36386457197198 0.971751831612376
3.29561769526148 0.985980195289496
3.24881431706591 1.00240644796764
3.20861244380214 1.01293429952561
3.16938767019224 1.02839853580769
3.18050056208889 1.05042831139707
3.16503509773993 1.08165869271809
3.208614253057 1.1164418127072
3.18412356131201 1.10544999991501
3.21190362926877 1.14284870029486
3.21027400805481 1.13248620425793
3.1700639722792 1.12856981396099
3.11517225580331 1.12136826430779
3.07335484285838 1.13975526380678
2.99570056124122 1.15118368116767
2.85846299112991 1.19951970322011
2.78757485262802 1.20221132249522
2.74221472731354 1.20186365755875
2.63435390947082 1.21033719632458
2.56660606991018 1.21925373592581
2.51794481030488 1.22002153597137
2.46911614289648 1.23972725018781
2.45058709697382 1.25168273938092
2.47135825381675 1.23057699533913
2.45283485458011 1.25793334385766
2.49496367430251 1.23861195945078
2.48904701255822 1.25862519873877
2.5646343025954 1.24417509580164
2.5687428966418 1.26722145795548
2.58730541323742 1.28285985998207
2.62251700243816 1.29433042920734
2.64333416476756 1.33602361791541
2.67948897550178 1.38722348527647
2.72166591565624 1.42740486735385
2.75270055594358 1.43096683264484
2.80677818151326 1.46420167865521
2.85133018420882 1.4606499087354
2.91066751505617 1.4628090494307
2.98482763034345 1.45993833472835
3.06730554673034 1.46263587920374
3.14460274091814 1.44949469574389
3.23213784635088 1.44062697468932
3.31024163079453 1.4270307741753
3.3512951091394 1.40036671651812
3.4017711046021 1.39766894649338
3.38549056476237 1.37806342977231
3.40526244113241 1.37318389131059
3.40346612365705 1.36299155725777
3.39371821855194 1.33984612380685
3.4019140630963 1.32903653727561
3.43280327400255 1.31918825508543
3.42039131920034 1.266029771924
3.47478814252454 1.23864452174203
3.52481279222092 1.20708994254779
3.59465430557435 1.14070726337675
3.64292121266644 1.11078098661924
3.71732876891936 1.04934668163039
3.78228755694404 1.02317563752568
3.84326397997338 0.97866913059187
3.87591104971136 0.953033900190684
3.90045321168651 0.941730769001205
3.91996780654539 0.928809906030269
3.89384541236475 0.928975172026874
3.8532622045896 0.908870429954832
3.8009317601632 0.906522072719271
3.747730859615 0.906822278537671
3.66707106515983 0.907357408886252
3.5915272141181 0.883460231704356
3.52093959907854 0.878559911280428
3.45350962038186 0.871585647476596
};
% \addlegendentry{Ours}
\addplot [line width=1pt, color0]
table {%
2.73138986085617 0.657010612239058
2.75360432320259 0.645698437987604
2.7508083515257 0.646742571562861
2.74550851348316 0.62647268601071
2.72250258307611 0.615033248815969
2.70890036336189 0.587527391166454
2.70048674867281 0.566557237876796
2.6621245905157 0.56724183290176
2.65258940451437 0.562835575197254
2.65388347721636 0.574767195104584
2.67367372667819 0.569375858413319
2.71430448120537 0.580960908636404
2.75246716597602 0.589230026100572
2.86294371432932 0.578972956710099
2.90622962533318 0.602869530796653
2.95056109235385 0.610498545305097
2.99364341688218 0.592091640957174
3.02859427991752 0.596601918924841
3.05303250126545 0.605446191691559
3.07371619488321 0.59331040534939
3.13888316455779 0.578954124385501
3.16026821946876 0.593471293840019
3.2011036391208 0.587441829084113
3.26194031975455 0.585436550167668
3.324686196072 0.574030825320271
3.39168199789358 0.583491131606597
3.45507064740115 0.590701699692942
3.54791406710348 0.565351407396609
3.56893738355065 0.569375888805397
3.57555290050113 0.573217204811524
3.58155283205009 0.578697321920415
3.54932629113885 0.558774371932346
3.53567629037423 0.570017814051165
3.51997284555271 0.580211876341465
3.433437696447 0.601787538331989
3.39377508547388 0.616557406612546
3.35114383424233 0.606157718175345
3.31313908978661 0.603748215910125
3.28820382358359 0.612260202930852
3.27425116100906 0.623836672256871
3.21557335445532 0.639473359682488
3.09517642619145 0.656413354814575
3.0237912725378 0.671493474375941
2.96730721438741 0.660581288371215
2.88654480121457 0.651813349136982
2.7825827012005 0.619723430507855
2.66926498137833 0.625654022015665
2.56055966975768 0.616804803660629
2.49794002158032 0.633532465778361
2.46771011458673 0.618005370455619
2.41016471761844 0.622471582166816
2.38746546621496 0.648487353780215
2.38373945569784 0.682968405146507
2.37568340169178 0.685387413787086
2.37438529736967 0.701568477070616
2.39164826922535 0.729654784320017
2.3902769834158 0.736487016563697
2.38948524431167 0.735191718975739
2.40738441948655 0.747989026078135
2.45310103488526 0.757754302568014
2.49340311007651 0.787481070169994
2.55163154853127 0.808336627680076
2.69675335918421 0.837018512573694
2.7828881224921 0.857900350992185
2.8781491291644 0.87983859016243
2.97401096266729 0.914689697777957
3.04490491628471 0.91779790983678
3.10674838697937 0.942201302549024
3.14268939458707 0.96160500839244
3.19304735985892 0.968176824179276
3.21979241206349 0.977424816005104
3.23261212494025 0.98854923733403
3.24157911978149 0.997481256467301
3.25282331608796 0.999000764258679
3.27531500357294 1.00551834148556
3.30946525165874 1.00210401950882
3.42385911017909 1.00202748043467
3.4925721935755 0.991707550655818
3.55868134397623 0.999853118029554
3.62211398508616 0.987300409123901
3.65590555658562 0.980690779878946
3.66762449416404 1.00865384311342
3.65635034189895 1.00505626919742
3.57450225759951 0.964686392024289
3.5158561928853 0.975173104382569
3.41539104845262 0.992214323705194
3.33620951102076 0.977635694403429
3.25981144745224 0.970582182546276
3.21774691837508 0.98772491904037
3.18190880196593 1.00187251057426
3.17415752571927 1.04332747828965
3.17693561005654 1.08104896882526
3.22823553566057 1.13409488077488
3.23357894433589 1.12385764666774
3.25220577008086 1.14058092021073
3.2515280013004 1.13862285041618
3.20585824063552 1.12637073288414
3.06770239653192 1.11237674535651
2.97668730023826 1.12632378485632
2.84576909514051 1.15338153706751
2.72324522445048 1.1802201492966
2.66511587162346 1.189201715826
2.56737987444208 1.18631715643634
2.49471329396189 1.19710683876199
2.4093239167304 1.20630857760943
2.39956970376416 1.21285429981377
2.4376903406125 1.202070126601
2.44608059076592 1.23690657263644
2.49113634814668 1.22873410169901
2.49765126578515 1.24007702537664
2.57138202453032 1.22883324088849
2.60142040165522 1.27584502213182
2.63148326539495 1.30200693519575
2.65489646110252 1.35019264639585
2.67590307732644 1.41278413765946
2.71555056669599 1.46554881335009
2.75553028398983 1.48216535325547
2.80934333571462 1.49711376504688
2.92733741621492 1.48416807027805
3.00795400936487 1.48239981199108
3.113924435822 1.48464560222221
3.20209421874616 1.47546689225864
3.29513009591462 1.46906545974477
3.37406738163484 1.45005143552191
3.41678144100867 1.42274324602061
3.42748138373125 1.39132730307169
3.41629296783595 1.3824463086832
3.39991136029194 1.36938887207413
3.38655207560852 1.34900145876894
3.38100526590359 1.33633294363003
3.41160372311744 1.32677290340083
3.42411932536854 1.29090759232864
3.46911867279182 1.24151728469815
3.62774585499471 1.14207346885956
3.68700583597362 1.10617092039616
3.76279959859637 1.04095998209618
3.83677982126538 1.01456959616795
3.89950867841041 0.997756247245787
3.93350333458381 0.968176820352702
3.94612092052851 0.962598085536201
3.90038448028181 0.967805219897478
3.83280522309102 0.969189952480515
3.75225049030137 0.956281648576645
3.67462506650057 0.96179460005697
3.57868141193329 0.973224968241479
3.48884590654207 0.945283145524123
3.33868769525814 0.928901271267334
3.27961156151381 0.909942415671177
3.24219519876619 0.906760277506214
};
% \addlegendentry{Point Cloud}
% \addplot [line width=1pt, green!50!black]
% table {%
% 2.79194092027163 0.675682647712128
% 2.79407119406988 0.703220041949035
% 2.79527527534208 0.711795270023535
% 2.79418461279521 0.726723723913668
% 2.7992917117979 0.727191847951841
% 2.81102871558341 0.713931684485897
% 2.79760860772589 0.702141990464947
% 2.78645569767935 0.677849089690324
% 2.75987040227934 0.655033487836737
% 2.74492820427677 0.622901863605389
% 2.73700166567946 0.58679370241161
% 2.71236227704775 0.564860313864813
% 2.68765841775157 0.564271594380181
% 2.67290493528827 0.559782760866558
% 2.66640708423765 0.565083992103844
% 2.67907644603627 0.555989880189345
% 2.71122620765581 0.563908618052208
% 2.73898108045827 0.569398247074381
% 2.78053817349636 0.560509803672526
% 2.83576546128013 0.56673625834506
% 2.86746986064176 0.591594042425316
% 2.90443960573929 0.60198713859095
% };
% \addlegendentry{Image}
\addplot [line width=1pt, black, dashed]
table {%
2.78004336357117 0.632818698883057
2.78473997116089 0.638318061828613
2.78169870376587 0.637591958045959
2.77279257774353 0.63290148973465
2.7611358165741 0.621461033821106
2.74732780456543 0.60774290561676
2.73093748092651 0.594337582588196
2.69390487670898 0.576365888118744
2.68285369873047 0.575522303581238
2.68129086494446 0.578539431095123
2.68994092941284 0.580935955047607
2.7073175907135 0.584364891052246
2.73254680633545 0.5893794298172
2.80578780174255 0.601789712905884
2.84787058830261 0.6033616065979
2.89023494720459 0.602049291133881
2.9271776676178 0.600774049758911
2.96092367172241 0.598361253738403
2.99176788330078 0.595715701580048
3.02260088920593 0.592634737491608
3.08351445198059 0.582817792892456
3.11538076400757 0.578564763069153
3.15450525283813 0.578361749649048
3.20232772827148 0.575249850749969
3.25803208351135 0.574694573879242
3.3161768913269 0.57064300775528
3.37219643592834 0.561338245868683
3.47152757644653 0.548518240451813
3.50878357887268 0.548225939273834
3.53404450416565 0.550397217273712
3.54474639892578 0.557612478733063
3.54177737236023 0.559260010719299
3.5278651714325 0.562194406986237
3.50693893432617 0.567442297935486
3.44325828552246 0.58589380979538
3.41175317764282 0.595011711120605
3.38133764266968 0.600455462932587
3.34080910682678 0.605159401893616
3.31128025054932 0.609150171279907
3.27819752693176 0.617089152336121
3.23718738555908 0.632509291172028
3.13333964347839 0.658334314823151
3.0713849067688 0.666970789432526
3.00010514259338 0.668299496173859
2.93614459037781 0.668152689933777
2.84673571586609 0.659588932991028
2.7660768032074 0.65624737739563
2.68826532363892 0.652865469455719
2.56908178329468 0.658845484256744
2.4967725276947 0.667507708072662
2.45544767379761 0.673418462276459
2.42531800270081 0.681628286838531
2.39972305297852 0.689211785793304
2.38822770118713 0.697850942611694
2.38112616539001 0.707625448703766
2.37244391441345 0.725314617156982
2.37436366081238 0.734794139862061
2.38197445869446 0.744607985019684
2.38410639762878 0.745479464530945
2.38410639762878 0.745479464530945
2.54188394546509 0.801227807998657
2.54188394546509 0.801227807998657
2.63489747047424 0.819602787494659
2.71523118019104 0.835769176483154
2.79587984085083 0.853483378887177
2.87371587753296 0.872008979320526
2.94537568092346 0.889821469783783
3.00989937782288 0.904130518436432
3.02894711494446 0.918487727642059
3.1410870552063 0.944109201431274
3.16888523101807 0.957380533218384
3.19266724586487 0.966566443443298
3.21331095695496 0.975494146347046
3.23522543907166 0.986978530883789
3.25612902641296 0.986358344554901
3.28694272041321 0.991490304470062
3.37403917312622 0.979946970939636
3.43747353553772 0.979255378246307
3.46730494499207 0.978964030742645
3.54685282707214 0.97417813539505
3.56150364875793 0.973176598548889
3.56150364875793 0.973176598548889
3.55420994758606 0.968668818473816
3.55420994758606 0.968668818473816
3.52897119522095 0.969216406345367
3.46123027801514 0.966148912906647
3.44793391227722 0.96590119600296
3.44793391227722 0.96590119600296
3.20479941368103 1.03704440593719
3.20479941368103 1.03704440593719
3.20333743095398 1.04014050960541
3.19610905647278 1.0569064617157
3.20433259010315 1.08610856533051
3.20877623558044 1.09527552127838
3.20877623558044 1.09527552127838
3.10875654220581 1.12826061248779
3.10875654220581 1.12826061248779
3.09200954437256 1.13175475597382
3.0337131023407 1.13904809951782
2.81984186172485 1.18516874313354
2.81984186172485 1.18516874313354
2.74672770500183 1.1967648267746
2.66049242019653 1.21030521392822
2.59113669395447 1.21736228466034
2.47602367401123 1.22587513923645
2.44892525672913 1.23063182830811
2.44124889373779 1.23750829696655
2.44737863540649 1.24806439876556
2.46477293968201 1.2597678899765
2.48559141159058 1.26518547534943
2.5109715461731 1.2717148065567
2.56022667884827 1.28673839569092
2.59123277664185 1.31957471370697
2.61795139312744 1.3553694486618
2.64434695243835 1.3904550075531
2.67542433738708 1.42694270610809
2.7141900062561 1.45624256134033
2.75917601585388 1.4771876335144
2.87690043449402 1.49541795253754
2.94824028015137 1.49557495117188
3.02909922599792 1.49183130264282
3.1125910282135 1.48014390468597
3.19374990463257 1.46717548370361
3.25704741477966 1.45282530784607
3.32147431373596 1.43851757049561
3.3886239528656 1.41326069831848
3.3969361782074 1.40173852443695
3.39630007743835 1.38950276374817
3.3953697681427 1.37267100811005
3.39798903465271 1.34983742237091
3.4073429107666 1.32186985015869
3.42936635017395 1.29361128807068
3.45953583717346 1.25897550582886
3.5581591129303 1.18452751636505
3.62155294418335 1.14020931720734
3.69111347198486 1.09253120422363
3.76070165634155 1.04756617546082
3.82333898544312 1.00902199745178
3.86648988723755 0.980598151683807
3.91346454620361 0.945891678333282
3.89978837966919 0.937991917133331
3.86199855804443 0.935832738876343
3.81219482421875 0.934732735157013
3.81219482421875 0.934732735157013
3.81219482421875 0.934732735157013
3.81219482421875 0.934732735157013
3.81219482421875 0.934732735157013
3.81219482421875 0.934732735157013
3.81219482421875 0.934732735157013
};
% \addlegendentry{GT}
\end{axis}

\end{tikzpicture}


==> tex/XYZ_plot/YZ_plot_seq3.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.188235294117647,0.188235294117647}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}


\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=white!80!black
},
axis line style= {white},
tick align=outside,
tick pos=left,
% title={XY plot},
xmajorgrids,
xmajorticks=true,
xminorgrids,
xminorgrids=true,
ymajorgrids,
ymajorticks=true,
yminorgrids,
yminorgrids=true,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
            minor tick num = 3,
        minor grid style={dashed},
x grid style={white!69.0196078431373!black},
xmin=2.12877276002231, xmax=5.16023554096054,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.404950771684837, ymax=1.54912152663555,
ytick style={color=black}
]
\addplot [line width=1pt, color1]
table {%
2.2954216427211 0.456958533273505
2.31777733333452 0.49487950715315
2.33763132237825 0.529290846679961
2.37099891932597 0.558159603164172
2.39915270681096 0.581603031021609
2.43237971210357 0.611786834903712
2.48228843678183 0.619828840130322
2.50723591521166 0.618996725006725
2.57016757457341 0.628498933188615
2.61110224606921 0.618617386776924
2.65472841443386 0.614607834975727
2.69645540690029 0.595761471537237
2.73302168382298 0.587547656728352
2.78460398196515 0.590958649413665
2.83162000452564 0.591881436489796
2.87356750945619 0.587976674053637
2.92110874032325 0.602002696201986
2.97777074365821 0.60076945794349
3.02254324868717 0.599485724584289
3.09168373521269 0.606668274298737
3.13921476015578 0.601798888398763
3.20421169494298 0.601803934405946
3.26403626073103 0.624994661038883
3.308839878853 0.618054264314445
3.35316934072594 0.633184133508421
3.39633428969372 0.621581680741958
3.43829247711476 0.608653774943656
3.47959461117091 0.575099462250055
3.50625344126635 0.572568446543079
3.52119343091084 0.572684579097422
3.55705093628962 0.582454008587114
3.58359333367066 0.572830630436128
3.61456898100191 0.57180452551432
3.66382379414986 0.591655611703931
3.70350267599603 0.601012115979793
3.73986772656383 0.597981792655272
3.79459211832735 0.583684884156747
3.8589167167674 0.588966843957799
3.92124063459251 0.59836364931814
3.99992257838136 0.597582087944079
4.04932519277265 0.593434769797821
4.12635767857896 0.595421832362148
4.18267360064715 0.587168678823642
4.26760867678425 0.61323269863585
4.33154077984819 0.619632582003686
4.40008314812554 0.616422580950774
4.44440381051309 0.642036095741194
4.50073852441353 0.627756915178666
4.54387388862518 0.600471148141839
4.57784565316582 0.616949772980762
4.61861403199193 0.638238638834733
4.65154330276112 0.644806702267674
4.64713122150596 0.63367921735363
4.65879743126192 0.669634341593406
4.70050728512957 0.689264916110825
4.71491058954871 0.670265382912131
4.66791998111957 0.673432023045431
4.66456338564272 0.663546258504555
4.6514615485341 0.673433980979231
4.61419404518564 0.658970398827948
4.57197420706711 0.666703837043153
4.53758470508788 0.671934417412527
4.46912709671841 0.653844414067499
4.42916135383894 0.65968524912859
4.34431157821041 0.685358084016413
4.25510880352394 0.69307586205989
4.19943957942588 0.701937000010989
4.10868519659685 0.720095622449483
4.03084815122655 0.724435974931953
3.96403028690104 0.731778433289824
3.87862436703802 0.741309372872078
3.81631763394191 0.734836655091209
3.75911789075354 0.761445802916635
3.71140899378346 0.759670298112906
3.65434881455194 0.789383693822738
3.60680009805964 0.803059543989636
3.58652056216466 0.813322396882952
3.55043822523879 0.824897819019936
3.53340288012352 0.840585453207842
3.52469800454746 0.849309565324545
3.52613146215501 0.879255694390182
3.50699401464921 0.87885509882795
3.54187917205913 0.904607260521757
3.53992240245697 0.911776331357928
3.55999978636447 0.926187070720048
3.58142860940515 0.934689504021621
3.59744380239372 0.933546064274718
3.61509018467778 0.954467023878263
3.64513837855198 0.966678058414332
3.67737153279367 0.956835685894477
3.70888977791336 0.973457766206282
3.76111119411413 0.976457955699481
3.81567450582051 0.978880187295118
3.87873492581653 0.978734109121055
3.94845073923546 0.96995812975022
4.00428374323119 0.97968247290656
4.07382113314224 0.964835905435578
4.13568268890664 0.963451033157929
4.22094809638009 0.995157931634678
4.28045051725409 0.972477292621147
4.35828816630771 0.951715788645927
4.4285547032453 0.95058415575198
4.47791919068106 0.960707664166411
4.55688852191186 0.984419651304546
4.62122417091992 0.971751831612376
4.68121848605205 0.985980195289496
4.73146398329164 1.00240644796764
4.78350441257105 1.01293429952561
4.83617557570634 1.02839853580769
4.88170283359478 1.05042831139707
4.93427000544225 1.08165869271809
4.95618168663791 1.1164418127072
4.95904613541331 1.10544999991501
4.97156268814394 1.14284870029486
4.96111937046137 1.13248620425793
4.95360187519411 1.12856981396099
4.94110527615339 1.12136826430779
4.90874431955096 1.13975526380678
4.88445928190409 1.15118368116767
4.84402526283237 1.19951970322011
4.81363791051145 1.20221132249522
4.74639621909141 1.20186365755875
4.70270904061743 1.21033719632458
4.64008299046569 1.21925373592581
4.57376563144212 1.22002153597137
4.49753014236375 1.23972725018781
4.4323391667904 1.25168273938092
4.3752508721595 1.23057699533913
4.30350269834918 1.25793334385766
4.23780888271187 1.23861195945078
4.16120874459902 1.25862519873877
4.08395576213948 1.24417509580164
3.99330635987506 1.26722145795548
3.90717893497241 1.28285985998207
3.82396238528935 1.29433042920734
3.73051040945206 1.33602361791541
3.67380135412162 1.38722348527647
3.62732310185697 1.42740486735385
3.60816445200711 1.43096683264484
3.6098946166593 1.46420167865521
3.62974614417943 1.4606499087354
3.63564250016771 1.4628090494307
3.67777015015346 1.45993833472835
3.71591579123588 1.46263587920374
3.75898147583426 1.44949469574389
3.79552346889038 1.44062697468932
3.82217176546725 1.4270307741753
3.85307696350958 1.40036671651812
3.88682844445628 1.39766894649338
3.88813003946867 1.37806342977231
3.89499281734444 1.37318389131059
3.89927045065691 1.36299155725777
3.86211921707423 1.33984612380685
3.8675035459905 1.32903653727561
3.8550389843343 1.31918825508543
3.84582553031054 1.266029771924
3.82192860675603 1.23864452174203
3.8188104365502 1.20708994254779
3.81326090765918 1.14070726337675
3.79713954466694 1.11078098661924
3.77813464376112 1.04934668163039
3.76760799931913 1.02317563752568
3.73444576200688 0.97866913059187
3.70009956408722 0.953033900190684
3.64725299707619 0.941730769001205
3.57459200766659 0.928809906030269
3.49507137704457 0.928975172026874
3.40462543050264 0.908870429954832
3.31878053771735 0.906522072719271
3.21306244747252 0.906822278537671
3.11988218513941 0.907357408886252
3.03607055697764 0.883460231704356
2.95875103539358 0.878559911280428
2.90943214434925 0.871585647476596
};
% \addlegendentry{Ours }
\addplot [line width=1pt, color0]
table {%
2.26656652279223 0.657010612239058
2.35714382130048 0.645698437987604
2.46912835587662 0.646742571562861
2.54904439484317 0.62647268601071
2.61610617873149 0.615033248815969
2.67091839597072 0.587527391166454
2.71293841304514 0.566557237876796
2.8289300166783 0.56724183290176
2.8774984141375 0.562835575197254
2.9297412196155 0.574767195104584
2.99582687673874 0.569375858413319
3.04398971125765 0.580960908636404
3.11821334733149 0.589230026100572
3.23500900778058 0.578972956710099
3.29710121648793 0.602869530796653
3.34523716767429 0.610498545305097
3.38133012793502 0.592091640957174
3.42218117361351 0.596601918924841
3.46468232077013 0.605446191691559
3.50232048035524 0.59331040534939
3.53138675226301 0.578954124385501
3.56050365837881 0.593471293840019
3.5866636872793 0.587441829084113
3.61679437274807 0.585436550167668
3.66508438167831 0.574030825320271
3.71110243709038 0.583491131606597
3.74881729731915 0.590701699692942
3.87321212722207 0.565351407396609
3.94332451694098 0.569375888805397
4.02933308877975 0.573217204811524
4.09019776487595 0.578697321920415
4.16508434190537 0.558774371932346
4.22440220256894 0.570017814051165
4.30491172300629 0.580211876341465
4.45110679138145 0.601787538331989
4.49818151091311 0.616557406612546
4.54490620065661 0.606157718175345
4.58474715181891 0.603748215910125
4.61732776598191 0.612260202930852
4.64513056496436 0.623836672256871
4.68209119320882 0.639473359682488
4.67689255581475 0.656413354814575
4.71121890184527 0.671493474375941
4.72908747193449 0.660581288371215
4.68988240652772 0.651813349136982
4.67061365107596 0.619723430507855
4.66318354414061 0.625654022015665
4.62011394913901 0.616804803660629
4.52897023159987 0.633532465778361
4.45192419369431 0.618005370455619
4.40100904910164 0.622471582166816
4.31615609623814 0.648487353780215
4.22276895453488 0.682968405146507
4.1513383273049 0.685387413787086
4.06132088987714 0.701568477070616
3.91240201883462 0.729654784320017
3.83365064700832 0.736487016563697
3.76827987219866 0.735191718975739
3.71381407610171 0.747989026078135
3.67536896327288 0.757754302568014
3.62523566406642 0.787481070169994
3.57816940186485 0.808336627680076
3.53342552792813 0.837018512573694
3.51982087848909 0.857900350992185
3.51785614866331 0.87983859016243
3.52830366103386 0.914689697777957
3.51297702842778 0.91779790983678
3.54607893560372 0.942201302549024
3.56705205771726 0.96160500839244
3.60401281076548 0.968176824179276
3.62928634441175 0.977424816005104
3.64446115856433 0.98854923733403
3.67286715948425 0.997481256467301
3.71002245775272 0.999000764258679
3.74868867147703 1.00551834148556
3.80102292687833 1.00210401950882
3.93236281040655 1.00202748043467
4.00647533265346 0.991707550655818
4.06658877149959 0.999853118029554
4.13244637976297 0.987300409123901
4.1961475001081 0.980690779878946
4.27739257805573 1.00865384311342
4.34797240131824 1.00505626919742
4.49815402389132 0.964686392024289
4.55318674767089 0.975173104382569
4.63109920128498 0.992214323705194
4.70003778680557 0.977635694403429
4.76173411000382 0.970582182546276
4.80983644276065 0.98772491904037
4.85795678179988 1.00187251057426
4.94957756098052 1.04332747828965
5.00200282074395 1.08104896882526
5.02244177819062 1.13409488077488
5.01361867542625 1.12385764666774
5.01083580216477 1.14058092021073
4.99080038985157 1.13862285041618
4.97426244268442 1.12637073288414
4.92098387821703 1.11237674535651
4.89068955830255 1.12632378485632
4.85105684806315 1.15338153706751
4.81949275852938 1.1802201492966
4.75215494766644 1.189201715826
4.7000965492915 1.18631715643634
4.6370482848981 1.19710683876199
4.48600491487912 1.20630857760943
4.4143954307876 1.21285429981377
4.35508778149186 1.202070126601
4.28856147136882 1.23690657263644
4.21924292669192 1.22873410169901
4.14232480811796 1.24007702537664
4.05807420954335 1.22883324088849
3.87004989365037 1.27584502213182
3.78420504498652 1.30200693519575
3.69286429381683 1.35019264639585
3.63283440896259 1.41278413765946
3.60052766507381 1.46554881335009
3.59385470673663 1.48216535325547
3.61573660602321 1.49711376504688
3.67854550142618 1.48416807027805
3.72883539212453 1.48239981199108
3.78066445016795 1.48464560222221
3.82685738124627 1.47546689225864
3.86869615050429 1.46906545974477
3.89120954533684 1.45005143552191
3.91382799082125 1.42274324602061
3.9365317018496 1.39132730307169
3.93210645408647 1.3824463086832
3.93231502623131 1.36938887207413
3.89157036167549 1.34900145876894
3.87612959104443 1.33633294363003
3.86039258272765 1.32677290340083
3.84920205010396 1.29090759232864
3.82223804415004 1.24151728469815
3.81118702895529 1.14207346885956
3.78918835850452 1.10617092039616
3.76273740012428 1.04095998209618
3.74379930250183 1.01456959616795
3.71244778006224 0.997756247245787
3.66098633321622 0.968176820352702
3.51781356500873 0.962598085536201
3.42482929034603 0.967805219897478
3.32435618429358 0.969189952480515
3.22850809599341 0.956281648576645
3.12001769870334 0.96179460005697
3.02508054511676 0.973224968241479
2.9409249519996 0.945283145524123
2.83436894351627 0.928901271267334
2.79343853460443 0.909942415671177
2.76691028471854 0.906760277506214
};
% \addlegendentry{Point Cloud}
% \addplot [line width=1pt, green!50!black]
% table {%
% 2.35892892452518 0.675682647712128
% 2.42978630582589 0.703220041949035
% 2.48453329989567 0.711795270023535
% 2.53544276599431 0.726723723913668
% 2.60163917930246 0.727191847951841
% 2.63961579753378 0.713931684485897
% 2.70738974953776 0.702141990464947
% 2.75855673276656 0.677849089690324
% 2.8035775783111 0.655033487836737
% 2.84376380208128 0.622901863605389
% 2.8750528381069 0.58679370241161
% 2.92158934911775 0.564860313864813
% 2.97520109740467 0.564271594380181
% 3.02040086164092 0.559782760866558
% 3.06965739993503 0.565083992103844
% 3.13503458401981 0.555989880189345
% 3.1852448045617 0.563908618052208
% 3.26139294599305 0.569398247074381
% 3.31810043051243 0.560509803672526
% 3.38685611116533 0.56673625834506
% 3.45422213542551 0.591594042425316
% 3.50698442114095 0.60198713859095
% };
% \addlegendentry{Image}
\addplot [line width=1pt, black, dashed]
table {%
2.44961881637573 0.632818698883057
2.49184632301331 0.638318061828613
2.53642201423645 0.637591958045959
2.5811128616333 0.63290148973465
2.62548923492432 0.621461033821106
2.66858124732971 0.60774290561676
2.71244502067566 0.594337582588196
2.80324053764343 0.576365888118744
2.84974360466003 0.575522303581238
2.89853239059448 0.578539431095123
2.95167922973633 0.580935955047607
3.00733399391174 0.584364891052246
3.06419110298157 0.5893794298172
3.17853021621704 0.601789712905884
3.23518180847168 0.6033616065979
3.28984522819519 0.602049291133881
3.34109807014465 0.600774049758911
3.38540554046631 0.598361253738403
3.42358613014221 0.595715701580048
3.4562566280365 0.592634737491608
3.50875163078308 0.582817792892456
3.53420877456665 0.578564763069153
3.55867266654968 0.578361749649048
3.58785653114319 0.575249850749969
3.6181046962738 0.574694573879242
3.65492224693298 0.57064300775528
3.70083785057068 0.561338245868683
3.80997467041016 0.548518240451813
3.87289643287659 0.548225939273834
3.93877172470093 0.550397217273712
4.00425100326538 0.557612478733063
4.07564973831177 0.559260010719299
4.14390993118286 0.562194406986237
4.21157598495483 0.567442297935486
4.34743690490723 0.58589380979538
4.3992977142334 0.595011711120605
4.44696283340454 0.600455462932587
4.50991916656494 0.605159401893616
4.55272197723389 0.609150171279907
4.59152603149414 0.617089152336121
4.62049102783203 0.632509291172028
4.66143894195557 0.658334314823151
4.67684459686279 0.666970789432526
4.68613862991333 0.668299496173859
4.68156385421753 0.668152689933777
4.67292547225952 0.659588932991028
4.65167999267578 0.65624737739563
4.62711381912231 0.652865469455719
4.56195640563965 0.658845484256744
4.48921155929565 0.667507708072662
4.42907476425171 0.673418462276459
4.364417552948 0.681628286838531
4.28832912445068 0.689211785793304
4.21258687973022 0.697850942611694
4.13534498214722 0.707625448703766
3.9815731048584 0.725314617156982
3.91040086746216 0.734794139862061
3.84459114074707 0.744607985019684
3.83271741867065 0.745479464530945
3.83271741867065 0.745479464530945
3.59143424034119 0.801227807998657
3.59143424034119 0.801227807998657
3.55322051048279 0.819602787494659
3.53378105163574 0.835769176483154
3.52052617073059 0.853483378887177
3.51484632492065 0.872008979320526
3.51649236679077 0.889821469783783
3.52600789070129 0.904130518436432
3.53686928749084 0.918487727642059
3.56351637840271 0.944109201431274
3.57629799842834 0.957380533218384
3.59665036201477 0.966566443443298
3.62381148338318 0.975494146347046
3.65565609931946 0.986978530883789
3.696049451828 0.986358344554901
3.73732781410217 0.991490304470062
3.84776592254639 0.979946970939636
3.91309595108032 0.979255378246307
3.94392347335815 0.978964030742645
4.03354120254517 0.97417813539505
4.05302429199219 0.973176598548889
4.05302429199219 0.973176598548889
4.41191577911377 0.968668818473816
4.41191577911377 0.968668818473816
4.44498062133789 0.969216406345367
4.51591968536377 0.966148912906647
4.52946996688843 0.96590119600296
4.52946996688843 0.96590119600296
4.8422794342041 1.03704440593719
4.8422794342041 1.03704440593719
4.84621095657349 1.04014050960541
4.88337802886963 1.0569064617157
4.92765474319458 1.08610856533051
4.93645238876343 1.09527552127838
4.93645238876343 1.09527552127838
4.93231248855591 1.12826061248779
4.93231248855591 1.12826061248779
4.92480373382568 1.13175475597382
4.9000825881958 1.13904809951782
4.80996656417847 1.18516874313354
4.80996656417847 1.18516874313354
4.77510261535645 1.1967648267746
4.72225284576416 1.21030521392822
4.67178773880005 1.21736228466034
4.53933477401733 1.22587513923645
4.4741735458374 1.23063182830811
4.4066367149353 1.23750829696655
4.33526086807251 1.24806439876556
4.2646312713623 1.2597678899765
4.19270467758179 1.26518547534943
4.11613798141479 1.2717148065567
3.95782518386841 1.28673839569092
3.86118698120117 1.31957471370697
3.78020834922791 1.3553694486618
3.71509742736816 1.3904550075531
3.66681861877441 1.42694270610809
3.63695573806763 1.45624256134033
3.62501287460327 1.4771876335144
3.65587210655212 1.49541795253754
3.68864607810974 1.49557495117188
3.72396874427795 1.49183130264282
3.75977635383606 1.48014390468597
3.79366683959961 1.46717548370361
3.82296109199524 1.45282530784607
3.85447812080383 1.43851757049561
3.89113712310791 1.41326069831848
3.89532256126404 1.40173852443695
3.89313435554504 1.38950276374817
3.88669848442078 1.37267100811005
3.8734872341156 1.34983742237091
3.85793447494507 1.32186985015869
3.84170961380005 1.29361128807068
3.82747554779053 1.25897550582886
3.80352425575256 1.18452751636505
3.7911856174469 1.14020931720734
3.77538084983826 1.09253120422363
3.75537896156311 1.04756617546082
3.72709131240845 1.00902199745178
3.69070506095886 0.980598151683807
3.56822967529297 0.945891678333282
3.49198365211487 0.937991917133331
3.40586566925049 0.935832738876343
3.32272267341614 0.934732735157013
3.32272267341614 0.934732735157013
3.32272267341614 0.934732735157013
3.32272267341614 0.934732735157013
3.32272267341614 0.934732735157013
3.32272267341614 0.934732735157013
3.32272267341614 0.934732735157013
};
% \addlegendentry{GT}
\end{axis}

\end{tikzpicture}


==> tex/error_seq/error_seq1.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{0.6,0,0.980392156862745}
% \definecolor{color1}{rgb}{0.968627450980392,0.00784313725490196,0.164705882352941}
% \definecolor{color2}{rgb}{0.0235294117647059,0.32156862745098,1}

\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
    legend cell align={left},
    legend style={
      fill opacity=0.8,
      draw opacity=1,
      text opacity=1,
      at={(-0.03,1.10)},
      anchor=north west,
      draw=white,
      /tikz/every even column/.append style={column sep=0.5cm},
    },
    legend columns=3,
    axis line style={white},
    tick align=outside,
    tick pos=left,
    % title={Seq 1 },
    x grid style={white!69.0196078431373!black},
    xmin=0.5, xmax=6.3,
    xtick style={color=black},
    xtick={1.4,3.4,5.4},
    xticklabels={X,Y,Z},
    y grid style={white!69.0196078431373!black},
    ylabel={ Error (m)},
    ymin=-0.0147050240191961, ymax=0.31,
    ytick style={color=black},
    xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
]

\draw[draw=color0,fill=color0, thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar, ybar legend, draw=color0,fill=color0,thick}
\addlegendentry{Tracking with only point cloud}

\draw[draw=color1,fill=color1, thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar, ybar legend, draw=color1,fill=color1,thick}
\addlegendentry{Tracking with only signal images}

\draw[draw=color2,fill=color2, thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar, ybar legend, draw=color2,fill=color2,thick}
\addlegendentry{Our approach}


\path [draw=color0, fill=color0]
(axis cs:0.9,0.0359016596706485)
--(axis cs:1.1,0.0359016596706485)
--(axis cs:1.1,0.123964853476531)
--(axis cs:0.9,0.123964853476531)
--(axis cs:0.9,0.0359016596706485)
--cycle;
\addplot [black, forget plot]
table {%
1 0.0359016596706485
1 0.000594158118181198
};
\addplot [black, forget plot]
table {%
1 0.123964853476531
1 0.219165955456631
};
\addplot [black, forget plot]
table {%
0.95 0.000594158118181198
1.05 0.000594158118181198
};
\addplot [black, forget plot]
table {%
0.95 0.219165955456631
1.05 0.219165955456631
};
\path [draw=color1, fill=color1]
(axis cs:1.3,0.0224564700129198)
--(axis cs:1.5,0.0224564700129198)
--(axis cs:1.5,0.131575909470591)
--(axis cs:1.3,0.131575909470591)
--(axis cs:1.3,0.0224564700129198)
--cycle;
\addplot [black, forget plot]
table {%
1.4 0.0224564700129198
1.4 0.00368735991092217
};
\addplot [black, forget plot]
table {%
1.4 0.131575909470591
1.4 0.177035822042366
};
\addplot [black, forget plot]
table {%
1.35 0.00368735991092217
1.45 0.00368735991092217
};
\addplot [black, forget plot]
table {%
1.35 0.177035822042366
1.45 0.177035822042366
};
\path [draw=color2, fill=color2]
(axis cs:1.7,0.00882856225400375)
--(axis cs:1.9,0.00882856225400375)
--(axis cs:1.9,0.0287960855190496)
--(axis cs:1.7,0.0287960855190496)
--(axis cs:1.7,0.00882856225400375)
--cycle;
\addplot [black, forget plot]
table {%
1.8 0.00882856225400375
1.8 0.000267686459507033
};
\addplot [black, forget plot]
table {%
1.8 0.0287960855190496
1.8 0.0584475453119366
};
\addplot [black, forget plot]
table {%
1.75 0.000267686459507033
1.85 0.000267686459507033
};
\addplot [black, forget plot]
table {%
1.75 0.0584475453119366
1.85 0.0584475453119366
};
\path [draw=color0, fill=color0]
(axis cs:2.9,0.0365788961205427)
--(axis cs:3.1,0.0365788961205427)
--(axis cs:3.1,0.0941762357336027)
--(axis cs:2.9,0.0941762357336027)
--(axis cs:2.9,0.0365788961205427)
--cycle;
\addplot [black, forget plot]
table {%
3 0.0365788961205427
3 0.000869162330838336
};
\addplot [black, forget plot]
table {%
3 0.0941762357336027
3 0.17826472756505
};
\addplot [black, forget plot]
table {%
2.95 0.000869162330838336
3.05 0.000869162330838336
};
\addplot [black, forget plot]
table {%
2.95 0.17826472756505
3.05 0.17826472756505
};
\path [draw=color1, fill=color1]
(axis cs:3.3,0.0936335797918026)
--(axis cs:3.5,0.0936335797918026)
--(axis cs:3.5,0.225292738533558)
--(axis cs:3.3,0.225292738533558)
--(axis cs:3.3,0.0936335797918026)
--cycle;
\addplot [black, forget plot]
table {%
3.4 0.0936335797918026
3.4 0.00413021189512097
};
\addplot [black, forget plot]
table {%
3.4 0.225292738533558
3.4 0.294725109117304
};
\addplot [black, forget plot]
table {%
3.35 0.00413021189512097
3.45 0.00413021189512097
};
\addplot [black, forget plot]
table {%
3.35 0.294725109117304
3.45 0.294725109117304
};
\path [draw=color2, fill=color2]
(axis cs:3.7,0.0105550124701859)
--(axis cs:3.9,0.0105550124701859)
--(axis cs:3.9,0.0439037283093395)
--(axis cs:3.7,0.0439037283093395)
--(axis cs:3.7,0.0105550124701859)
--cycle;
\addplot [black, forget plot]
table {%
3.8 0.0105550124701859
3.8 0.000138631389560828
};
\addplot [black, forget plot]
table {%
3.8 0.0439037283093395
3.8 0.0823405821542753
};
\addplot [black, forget plot]
table {%
3.75 0.000138631389560828
3.85 0.000138631389560828
};
\addplot [black, forget plot]
table {%
3.75 0.0823405821542753
3.85 0.0823405821542753
};
\path [draw=color0, fill=color0]
(axis cs:4.9,0.0255128619703696)
--(axis cs:5.1,0.0255128619703696)
--(axis cs:5.1,0.0756290965564553)
--(axis cs:4.9,0.0756290965564553)
--(axis cs:4.9,0.0255128619703696)
--cycle;
\addplot [black, forget plot]
table {%
5 0.0255128619703696
5 0.00148441613567574
};
\addplot [black, forget plot]
table {%
5 0.0756290965564553
5 0.148283764805501
};
\addplot [black, forget plot]
table {%
4.95 0.00148441613567574
5.05 0.00148441613567574
};
\addplot [black, forget plot]
table {%
4.95 0.148283764805501
5.05 0.148283764805501
};
\path [draw=color1, fill=color1]
(axis cs:5.3,0.00532853403802855)
--(axis cs:5.5,0.00532853403802855)
--(axis cs:5.5,0.0127842448158017)
--(axis cs:5.3,0.0127842448158017)
--(axis cs:5.3,0.00532853403802855)
--cycle;
\addplot [black, forget plot]
table {%
5.4 0.00532853403802855
5.4 0.00142377354419265
};
\addplot [black, forget plot]
table {%
5.4 0.0127842448158017
5.4 0.0237795656365393
};
\addplot [black, forget plot]
table {%
5.35 0.00142377354419265
5.45 0.00142377354419265
};
\addplot [black, forget plot]
table {%
5.35 0.0237795656365393
5.45 0.0237795656365393
};
\path [draw=color2, fill=color2]
(axis cs:5.7,0.00727972918056854)
--(axis cs:5.9,0.00727972918056854)
--(axis cs:5.9,0.0231674857426256)
--(axis cs:5.7,0.0231674857426256)
--(axis cs:5.7,0.00727972918056854)
--cycle;
\addplot [black, forget plot]
table {%
5.8 0.00727972918056854
5.8 2.9744225399142e-05
};
\addplot [black, forget plot]
table {%
5.8 0.0231674857426256
5.8 0.0459741988826368
};
\addplot [black, forget plot]
table {%
5.75 2.9744225399142e-05
5.85 2.9744225399142e-05
};
\addplot [black, forget plot]
table {%
5.75 0.0459741988826368
5.85 0.0459741988826368
};
\addplot [line width=1pt, white, forget plot]
table {%
0.9 0.0765784603353681
1.1 0.0765784603353681
};
\addplot [line width=1pt, white, forget plot]
table {%
1.3 0.0798680383669237
1.5 0.0798680383669237
};
\addplot [line width=1pt, white, forget plot]
table {%
1.7 0.0167689702781684
1.9 0.0167689702781684
};
\addplot [line width=1pt, white, forget plot]
table {%
2.9 0.0651368712573408
3.1 0.0651368712573408
};
\addplot [line width=1pt, white, forget plot]
table {%
3.3 0.167468870553379
3.5 0.167468870553379
};
\addplot [line width=1pt, white, forget plot]
table {%
3.7 0.0247040115872634
3.9 0.0247040115872634
};
\addplot [line width=1pt, white, forget plot]
table {%
4.9 0.0489386840818955
5.1 0.0489386840818955
};
\addplot [line width=1pt, white, forget plot]
table {%
5.3 0.00967427726703923
5.5 0.00967427726703923
};
\addplot [line width=1pt, white, forget plot]
table {%
5.7 0.0139552293806988
5.9 0.0139552293806988
};
\end{axis}

\end{tikzpicture}


==> tex/error_seq/error_seq2.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{0.6,0,0.980392156862745}
% \definecolor{color1}{rgb}{0.968627450980392,0.00784313725490196,0.164705882352941}
% \definecolor{color2}{rgb}{0.0235294117647059,0.32156862745098,1}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
    legend cell align={left},
    legend style={
      fill opacity=0.8,
      draw opacity=1,
      text opacity=1,
      at={(0.03,0.97)},
      anchor=north west,
      draw=white!80!black
    },
axis line style={white},
tick align=outside,
tick pos=left,
% title={Seq 2 },
x grid style={white!69.0196078431373!black},
xmin=0.5, xmax=6.3,
xtick style={color=black},
xtick={1.4,3.4,5.4},
xticklabels={X,Y,Z},
y grid style={white!69.0196078431373!black},
ylabel={ Error (m)},
ymin=-0.00876739680516033, ymax=0.184969536254822,
ytick style={color=black},
    xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
]
\path [draw=color0, fill=color0]
(axis cs:0.9,0.00815245852515445)
--(axis cs:1.1,0.00815245852515445)
--(axis cs:1.1,0.0355660872611989)
--(axis cs:0.9,0.0355660872611989)
--(axis cs:0.9,0.00815245852515445)
--cycle;
\addplot [black, forget plot]
table {%
1 0.00815245852515445
1 0.000677464621831714
};
\addplot [black, forget plot]
table {%
1 0.0355660872611989
1 0.0760465676788473
};
\addplot [black, forget plot]
table {%
0.95 0.000677464621831714
1.05 0.000677464621831714
};
\addplot [black, forget plot]
table {%
0.95 0.0760465676788473
1.05 0.0760465676788473
};
\path [draw=color1, fill=color1]
(axis cs:1.3,0.00430830867868714)
--(axis cs:1.5,0.00430830867868714)
--(axis cs:1.5,0.0151839841291762)
--(axis cs:1.3,0.0151839841291762)
--(axis cs:1.3,0.00430830867868714)
--cycle;
\addplot [black, forget plot]
table {%
1.4 0.00430830867868714
1.4 0.0010557370823836
};
\addplot [black, forget plot]
table {%
1.4 0.0151839841291762
1.4 0.0231649600846127
};
\addplot [black, forget plot]
table {%
1.35 0.0010557370823836
1.45 0.0010557370823836
};
\addplot [black, forget plot]
table {%
1.35 0.0231649600846127
1.45 0.0231649600846127
};
\path [draw=color2, fill=color2]
(axis cs:1.7,0.0108070949987866)
--(axis cs:1.9,0.0108070949987866)
--(axis cs:1.9,0.0469455026016019)
--(axis cs:1.7,0.0469455026016019)
--(axis cs:1.7,0.0108070949987866)
--cycle;
\addplot [black, forget plot]
table {%
1.8 0.0108070949987866
1.8 3.88274248388498e-05
};
\addplot [black, forget plot]
table {%
1.8 0.0469455026016019
1.8 0.0722655397008891
};
\addplot [black, forget plot]
table {%
1.75 3.88274248388498e-05
1.85 3.88274248388498e-05
};
\addplot [black, forget plot]
table {%
1.75 0.0722655397008891
1.85 0.0722655397008891
};
\path [draw=color0, fill=color0]
(axis cs:2.9,0.00974226341835482)
--(axis cs:3.1,0.00974226341835482)
--(axis cs:3.1,0.0424458183453618)
--(axis cs:2.9,0.0424458183453618)
--(axis cs:2.9,0.00974226341835482)
--cycle;
\addplot [black, forget plot]
table {%
3 0.00974226341835482
3 0.0003648774884768
};
\addplot [black, forget plot]
table {%
3 0.0424458183453618
3 0.0759341926763533
};
\addplot [black, forget plot]
table {%
2.95 0.0003648774884768
3.05 0.0003648774884768
};
\addplot [black, forget plot]
table {%
2.95 0.0759341926763533
3.05 0.0759341926763533
};
\path [draw=color1, fill=color1]
(axis cs:3.3,0.0336190006785358)
--(axis cs:3.5,0.0336190006785358)
--(axis cs:3.5,0.097577699413025)
--(axis cs:3.3,0.097577699413025)
--(axis cs:3.3,0.0336190006785358)
--cycle;
\addplot [black, forget plot]
table {%
3.4 0.0336190006785358
3.4 0.0030644107688782
};
\addplot [black, forget plot]
table {%
3.4 0.097577699413025
3.4 0.176163312024822
};
\addplot [black, forget plot]
table {%
3.35 0.0030644107688782
3.45 0.0030644107688782
};
\addplot [black, forget plot]
table {%
3.35 0.176163312024822
3.45 0.176163312024822
};
\path [draw=color2, fill=color2]
(axis cs:3.7,0.00808186866347871)
--(axis cs:3.9,0.00808186866347871)
--(axis cs:3.9,0.0440748566983342)
--(axis cs:3.7,0.0440748566983342)
--(axis cs:3.7,0.00808186866347871)
--cycle;
\addplot [black, forget plot]
table {%
3.8 0.00808186866347871
3.8 0.0001008556550679
};
\addplot [black, forget plot]
table {%
3.8 0.0440748566983342
3.8 0.0881248202830607
};
\addplot [black, forget plot]
table {%
3.75 0.0001008556550679
3.85 0.0001008556550679
};
\addplot [black, forget plot]
table {%
3.75 0.0881248202830607
3.85 0.0881248202830607
};
\path [draw=color0, fill=color0]
(axis cs:4.9,0.00612243655419784)
--(axis cs:5.1,0.00612243655419784)
--(axis cs:5.1,0.0209237401912207)
--(axis cs:4.9,0.0209237401912207)
--(axis cs:4.9,0.00612243655419784)
--cycle;
\addplot [black, forget plot]
table {%
5 0.00612243655419784
5 0.000388261695153491
};
\addplot [black, forget plot]
table {%
5 0.0209237401912207
5 0.0392731995430584
};
\addplot [black, forget plot]
table {%
4.95 0.000388261695153491
5.05 0.000388261695153491
};
\addplot [black, forget plot]
table {%
4.95 0.0392731995430584
5.05 0.0392731995430584
};
\path [draw=color1, fill=color1]
(axis cs:5.3,0.0139338719068252)
--(axis cs:5.5,0.0139338719068252)
--(axis cs:5.5,0.040402023571507)
--(axis cs:5.3,0.040402023571507)
--(axis cs:5.3,0.0139338719068252)
--cycle;
\addplot [black, forget plot]
table {%
5.4 0.0139338719068252
5.4 0.00455167088083763
};
\addplot [black, forget plot]
table {%
5.4 0.040402023571507
5.4 0.065507495128893
};
\addplot [black, forget plot]
table {%
5.35 0.00455167088083763
5.45 0.00455167088083763
};
\addplot [black, forget plot]
table {%
5.35 0.065507495128893
5.45 0.065507495128893
};
\path [draw=color2, fill=color2]
(axis cs:5.7,0.004761184148176)
--(axis cs:5.9,0.004761184148176)
--(axis cs:5.9,0.0178303404227792)
--(axis cs:5.7,0.0178303404227792)
--(axis cs:5.7,0.004761184148176)
--cycle;
\addplot [black, forget plot]
table {%
5.8 0.004761184148176
5.8 0.000167742242199065
};
\addplot [black, forget plot]
table {%
5.8 0.0178303404227792
5.8 0.0364272724509153
};
\addplot [black, forget plot]
table {%
5.75 0.000167742242199065
5.85 0.000167742242199065
};
\addplot [black, forget plot]
table {%
5.75 0.0364272724509153
5.85 0.0364272724509153
};
\addplot [line width=1pt, white, forget plot]
table {%
0.9 0.0202748343545978
1.1 0.0202748343545978
};
\addplot [line width=1pt, white, forget plot]
table {%
1.3 0.00982938124535071
1.5 0.00982938124535071
};
\addplot [line width=1pt, white, forget plot]
table {%
1.7 0.029147362000046
1.9 0.029147362000046
};
\addplot [line width=1pt, white, forget plot]
table {%
2.9 0.0267552841689922
3.1 0.0267552841689922
};
\addplot [line width=1pt, white, forget plot]
table {%
3.3 0.0701316623582899
3.5 0.0701316623582899
};
\addplot [line width=1pt, white, forget plot]
table {%
3.7 0.0192756859440788
3.9 0.0192756859440788
};
\addplot [line width=1pt, white, forget plot]
table {%
4.9 0.0129318118170228
5.1 0.0129318118170228
};
\addplot [line width=1pt, white, forget plot]
table {%
5.3 0.0231806449570045
5.5 0.0231806449570045
};
\addplot [line width=1pt, white, forget plot]
table {%
5.7 0.0113959344884098
5.9 0.0113959344884098
};
\end{axis}

\end{tikzpicture}


==> tex/error_seq/error_seq3.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{0.6,0,0.980392156862745}
% \definecolor{color1}{rgb}{0.968627450980392,0.00784313725490196,0.164705882352941}
% \definecolor{color2}{rgb}{0.0235294117647059,0.32156862745098,1}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}


\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
    legend cell align={left},
    legend style={
      fill opacity=0.8,
      draw opacity=1,
      text opacity=1,
      at={(0.03,0.97)},
      anchor=north west,
      draw=white!80!black
    },
axis line style={white},
tick align=outside,
tick pos=left,
% title={Seq 3 },
x grid style={white!69.0196078431373!black},
xmin=0.5, xmax=6.3,
xtick style={color=black},
xtick={1.4,3.4,5.4},
xticklabels={X,Y,Z},
y grid style={white!69.0196078431373!black},
ylabel={ Error (m)},
ymin=-0.00897775582982006, ymax=0.189937849485646,
ytick style={color=black},
        xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
]
\path [draw=color0, fill=color0]
(axis cs:0.9,0.0232780218577666)
--(axis cs:1.1,0.0232780218577666)
--(axis cs:1.1,0.0711417617143559)
--(axis cs:0.9,0.0711417617143559)
--(axis cs:0.9,0.0232780218577666)
--cycle;
\addplot [black, forget plot]
table {%
1 0.0232780218577666
1 0.000596100612618056
};
\addplot [black, forget plot]
table {%
1 0.0711417617143559
1 0.142771459094593
};
\addplot [black, forget plot]
table {%
0.95 0.000596100612618056
1.05 0.000596100612618056
};
\addplot [black, forget plot]
table {%
0.95 0.142771459094593
1.05 0.142771459094593
};
\path [draw=color1, fill=color1]
(axis cs:1.3,0.0088396449768362)
--(axis cs:1.5,0.0088396449768362)
--(axis cs:1.5,0.0177479663700559)
--(axis cs:1.3,0.0177479663700559)
--(axis cs:1.3,0.0088396449768362)
--cycle;
\addplot [black, forget plot]
table {%
1.4 0.0088396449768362
1.4 0.000359157874370908
};
\addplot [black, forget plot]
table {%
1.4 0.0177479663700559
1.4 0.0278344120708334
};
\addplot [black, forget plot]
table {%
1.35 0.000359157874370908
1.45 0.000359157874370908
};
\addplot [black, forget plot]
table {%
1.35 0.0278344120708334
1.45 0.0278344120708334
};
\path [draw=color2, fill=color2]
(axis cs:1.7,0.0114199810676545)
--(axis cs:1.9,0.0114199810676545)
--(axis cs:1.9,0.053081363686204)
--(axis cs:1.7,0.053081363686204)
--(axis cs:1.7,0.0114199810676545)
--cycle;
\addplot [black, forget plot]
table {%
1.8 0.0114199810676545
1.8 0.000901600574375827
};
\addplot [black, forget plot]
table {%
1.8 0.053081363686204
1.8 0.108638698498432
};
\addplot [black, forget plot]
table {%
1.75 0.000901600574375827
1.85 0.000901600574375827
};
\addplot [black, forget plot]
table {%
1.75 0.108638698498432
1.85 0.108638698498432
};
\path [draw=color0, fill=color0]
(axis cs:2.9,0.0279910207296199)
--(axis cs:3.1,0.0279910207296199)
--(axis cs:3.1,0.0771662866628215)
--(axis cs:2.9,0.0771662866628215)
--(axis cs:2.9,0.0279910207296199)
--cycle;
\addplot [black, forget plot]
table {%
3 0.0279910207296199
3 0.000493392369484091
};
\addplot [black, forget plot]
table {%
3 0.0771662866628215
3 0.14312320811591
};
\addplot [black, forget plot]
table {%
2.95 0.000493392369484091
3.05 0.000493392369484091
};
\addplot [black, forget plot]
table {%
2.95 0.14312320811591
3.05 0.14312320811591
};
\path [draw=color1, fill=color1]
(axis cs:3.3,0.133592629973776)
--(axis cs:3.5,0.133592629973776)
--(axis cs:3.5,0.1742756192671)
--(axis cs:3.3,0.1742756192671)
--(axis cs:3.3,0.133592629973776)
--cycle;
\addplot [black, forget plot]
table {%
3.4 0.133592629973776
3.4 0.0787552872431321
};
\addplot [black, forget plot]
table {%
3.4 0.1742756192671
3.4 0.180896231062216
};
\addplot [black, forget plot]
table {%
3.35 0.0787552872431321
3.45 0.0787552872431321
};
\addplot [black, forget plot]
table {%
3.35 0.180896231062216
3.45 0.180896231062216
};
\path [draw=color2, fill=color2]
(axis cs:3.7,0.0143334506366791)
--(axis cs:3.9,0.0143334506366791)
--(axis cs:3.9,0.0484907984263832)
--(axis cs:3.7,0.0484907984263832)
--(axis cs:3.7,0.0143334506366791)
--cycle;
\addplot [black, forget plot]
table {%
3.8 0.0143334506366791
3.8 0.00152332401541067
};
\addplot [black, forget plot]
table {%
3.8 0.0484907984263832
3.8 0.0919856255534661
};
\addplot [black, forget plot]
table {%
3.75 0.00152332401541067
3.85 0.00152332401541067
};
\addplot [black, forget plot]
table {%
3.75 0.0919856255534661
3.85 0.0919856255534661
};
\path [draw=color0, fill=color0]
(axis cs:4.9,0.00718570042061395)
--(axis cs:5.1,0.00718570042061395)
--(axis cs:5.1,0.02510844997279)
--(axis cs:4.9,0.02510844997279)
--(axis cs:4.9,0.00718570042061395)
--cycle;
\addplot [black, forget plot]
table {%
5 0.00718570042061395
5 0.000149403716627639
};
\addplot [black, forget plot]
table {%
5 0.02510844997279
5 0.0515712221274507
};
\addplot [black, forget plot]
table {%
4.95 0.000149403716627639
5.05 0.000149403716627639
};
\addplot [black, forget plot]
table {%
4.95 0.0515712221274507
5.05 0.0515712221274507
};
\path [draw=color1, fill=color1]
(axis cs:5.3,0.016524061983732)
--(axis cs:5.5,0.016524061983732)
--(axis cs:5.5,0.0702343830365995)
--(axis cs:5.3,0.0702343830365995)
--(axis cs:5.3,0.016524061983732)
--cycle;
\addplot [black, forget plot]
table {%
5.4 0.016524061983732
5.4 0.00088228305353566
};
\addplot [black, forget plot]
table {%
5.4 0.0702343830365995
5.4 0.136660089747208
};
\addplot [black, forget plot]
table {%
5.35 0.00088228305353566
5.45 0.00088228305353566
};
\addplot [black, forget plot]
table {%
5.35 0.136660089747208
5.45 0.136660089747208
};
\path [draw=color2, fill=color2]
(axis cs:5.7,0.00499251809664381)
--(axis cs:5.9,0.00499251809664381)
--(axis cs:5.9,0.0189492854816761)
--(axis cs:5.7,0.0189492854816761)
--(axis cs:5.7,0.00499251809664381)
--cycle;
\addplot [black, forget plot]
table {%
5.8 0.00499251809664381
5.8 6.38625936102422e-05
};
\addplot [black, forget plot]
table {%
5.8 0.0189492854816761
5.8 0.0394391370956968
};
\addplot [black, forget plot]
table {%
5.75 6.38625936102422e-05
5.85 6.38625936102422e-05
};
\addplot [black, forget plot]
table {%
5.75 0.0394391370956968
5.85 0.0394391370956968
};
\addplot [line width=1pt, white, forget plot]
table {%
0.9 0.0452829561791654
1.1 0.0452829561791654
};
\addplot [line width=1pt, white, forget plot]
table {%
1.3 0.0120809718295072
1.5 0.0120809718295072
};
\addplot [line width=1pt, white, forget plot]
table {%
1.7 0.0255258806510643
1.9 0.0255258806510643
};
\addplot [line width=1pt, white, forget plot]
table {%
2.9 0.0515489334434402
3.1 0.0515489334434402
};
\addplot [line width=1pt, white, forget plot]
table {%
3.3 0.14480473897281
3.5 0.14480473897281
};
\addplot [line width=1pt, white, forget plot]
table {%
3.7 0.025519191420708
3.9 0.025519191420708
};
\addplot [line width=1pt, white, forget plot]
table {%
4.9 0.0157743244749928
5.1 0.0157743244749928
};
\addplot [line width=1pt, white, forget plot]
table {%
5.3 0.0370830731462402
5.5 0.0370830731462402
};
\addplot [line width=1pt, white, forget plot]
table {%
5.7 0.00942297550400267
5.9 0.00942297550400267
};
\end{axis}

\end{tikzpicture}


==> tex/velo_error_seq/velo_error_seq1.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{0.6,0,0.980392156862745}
% \definecolor{color1}{rgb}{0.968627450980392,0.00784313725490196,0.164705882352941}
% \definecolor{color2}{rgb}{0.0235294117647059,0.32156862745098,1}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(-0.03,1.12)},
  anchor=north west,
  draw=white,
/tikz/every even column/.append style={column sep=0.5cm},
},
legend columns = 3, 
axis line style={white},
tick align=outside,
tick pos=left,
% title={Seq 1 },
x grid style={white!69.0196078431373!black},
xmin=0.5, xmax=6.3,
xtick style={color=black},
xtick={1.4,3.4,5.4},
xticklabels={X,Y,Z},
y grid style={white!69.0196078431373!black},
ylabel={Velocity Error (m/s)},
ymin=-0.034208951695738, ymax=0.721221921251871,
ytick style={color=black},
    xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
]

\draw[draw=color0,fill=color0, thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar, ybar legend, draw=color0,fill=color0,thick}
\addlegendentry{Tracking with only point cloud}

\draw[draw=color1,fill=color1, thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar, ybar legend, draw=color1,fill=color1,thick}
\addlegendentry{Tracking with only signal images}

\draw[draw=color2,fill=color2, thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar, ybar legend, draw=color2,fill=color2,thick}
\addlegendentry{Our approach}

\path [draw=color0, fill=color0]
(axis cs:0.9,0.109162671124885)
--(axis cs:1.1,0.109162671124885)
--(axis cs:1.1,0.344490432716165)
--(axis cs:0.9,0.344490432716165)
--(axis cs:0.9,0.109162671124885)
--cycle;
\addplot [black, forget plot]
table {%
1 0.109162671124885
1 0.000128815256426051
};
\addplot [black, forget plot]
table {%
1 0.344490432716165
1 0.686884154299707
};
\addplot [black, forget plot]
table {%
0.95 0.000128815256426051
1.05 0.000128815256426051
};
\addplot [black, forget plot]
table {%
0.95 0.686884154299707
1.05 0.686884154299707
};
\path [draw=color1, fill=color1]
(axis cs:1.3,0.0919291443556336)
--(axis cs:1.5,0.0919291443556336)
--(axis cs:1.5,0.24845085936301)
--(axis cs:1.3,0.24845085936301)
--(axis cs:1.3,0.0919291443556336)
--cycle;
\addplot [black, forget plot]
table {%
1.4 0.0919291443556336
1.4 0.00361160361343593
};
\addplot [black, forget plot]
table {%
1.4 0.24845085936301
1.4 0.392370148027017
};
\addplot [black, forget plot]
table {%
1.35 0.00361160361343593
1.45 0.00361160361343593
};
\addplot [black, forget plot]
table {%
1.35 0.392370148027017
1.45 0.392370148027017
};
\path [draw=color2, fill=color2]
(axis cs:1.7,0.0651457039411474)
--(axis cs:1.9,0.0651457039411474)
--(axis cs:1.9,0.248436061039956)
--(axis cs:1.7,0.248436061039956)
--(axis cs:1.7,0.0651457039411474)
--cycle;
\addplot [black, forget plot]
table {%
1.8 0.0651457039411474
1.8 0.0027373277432563
};
\addplot [black, forget plot]
table {%
1.8 0.248436061039956
1.8 0.493909091734377
};
\addplot [black, forget plot]
table {%
1.75 0.0027373277432563
1.85 0.0027373277432563
};
\addplot [black, forget plot]
table {%
1.75 0.493909091734377
1.85 0.493909091734377
};
\path [draw=color0, fill=color0]
(axis cs:2.9,0.0771871383898404)
--(axis cs:3.1,0.0771871383898404)
--(axis cs:3.1,0.347491246148062)
--(axis cs:2.9,0.347491246148062)
--(axis cs:2.9,0.0771871383898404)
--cycle;
\addplot [black, forget plot]
table {%
3 0.0771871383898404
3 0.000199890722223373
};
\addplot [black, forget plot]
table {%
3 0.347491246148062
3 0.677734254757247
};
\addplot [black, forget plot]
table {%
2.95 0.000199890722223373
3.05 0.000199890722223373
};
\addplot [black, forget plot]
table {%
2.95 0.677734254757247
3.05 0.677734254757247
};
\path [draw=color1, fill=color1]
(axis cs:3.3,0.158876445092808)
--(axis cs:3.5,0.158876445092808)
--(axis cs:3.5,0.366330405403881)
--(axis cs:3.3,0.366330405403881)
--(axis cs:3.3,0.158876445092808)
--cycle;
\addplot [black, forget plot]
table {%
3.4 0.158876445092808
3.4 0.0153142890715063
};
\addplot [black, forget plot]
table {%
3.4 0.366330405403881
3.4 0.486702403844719
};
\addplot [black, forget plot]
table {%
3.35 0.0153142890715063
3.45 0.0153142890715063
};
\addplot [black, forget plot]
table {%
3.35 0.486702403844719
3.45 0.486702403844719
};
\path [draw=color2, fill=color2]
(axis cs:3.7,0.0411681137598663)
--(axis cs:3.9,0.0411681137598663)
--(axis cs:3.9,0.163136180242405)
--(axis cs:3.7,0.163136180242405)
--(axis cs:3.7,0.0411681137598663)
--cycle;
\addplot [black, forget plot]
table {%
3.8 0.0411681137598663
3.8 0.000443114872510364
};
\addplot [black, forget plot]
table {%
3.8 0.163136180242405
3.8 0.342459269664861
};
\addplot [black, forget plot]
table {%
3.75 0.000443114872510364
3.85 0.000443114872510364
};
\addplot [black, forget plot]
table {%
3.75 0.342459269664861
3.85 0.342459269664861
};
\path [draw=color0, fill=color0]
(axis cs:4.9,0.070570502146341)
--(axis cs:5.1,0.070570502146341)
--(axis cs:5.1,0.276398234476372)
--(axis cs:4.9,0.276398234476372)
--(axis cs:4.9,0.070570502146341)
--cycle;
\addplot [black, forget plot]
table {%
5 0.070570502146341
5 0.000259953570465044
};
\addplot [black, forget plot]
table {%
5 0.276398234476372
5 0.531454865660448
};
\addplot [black, forget plot]
table {%
4.95 0.000259953570465044
5.05 0.000259953570465044
};
\addplot [black, forget plot]
table {%
4.95 0.531454865660448
5.05 0.531454865660448
};
\path [draw=color1, fill=color1]
(axis cs:5.3,0.0136535369876245)
--(axis cs:5.5,0.0136535369876245)
--(axis cs:5.5,0.0975762615115577)
--(axis cs:5.3,0.0975762615115577)
--(axis cs:5.3,0.0136535369876245)
--cycle;
\addplot [black, forget plot]
table {%
5.4 0.0136535369876245
5.4 0.00456348111469773
};
\addplot [black, forget plot]
table {%
5.4 0.0975762615115577
5.4 0.209099309075048
};
\addplot [black, forget plot]
table {%
5.35 0.00456348111469773
5.45 0.00456348111469773
};
\addplot [black, forget plot]
table {%
5.35 0.209099309075048
5.45 0.209099309075048
};
\path [draw=color2, fill=color2]
(axis cs:5.7,0.051383654669091)
--(axis cs:5.9,0.051383654669091)
--(axis cs:5.9,0.210674396423683)
--(axis cs:5.7,0.210674396423683)
--(axis cs:5.7,0.051383654669091)
--cycle;
\addplot [black, forget plot]
table {%
5.8 0.051383654669091
5.8 0.000249636769975581
};
\addplot [black, forget plot]
table {%
5.8 0.210674396423683
5.8 0.438200065621051
};
\addplot [black, forget plot]
table {%
5.75 0.000249636769975581
5.85 0.000249636769975581
};
\addplot [black, forget plot]
table {%
5.75 0.438200065621051
5.85 0.438200065621051
};
\addplot [line width=1pt, white, forget plot]
table {%
0.9 0.191737841303157
1.1 0.191737841303157
};
\addplot [line width=1pt, white, forget plot]
table {%
1.3 0.197800169460929
1.5 0.197800169460929
};
\addplot [line width=1pt, white, forget plot]
table {%
1.7 0.128881545706658
1.9 0.128881545706658
};
\addplot [line width=1pt, white, forget plot]
table {%
2.9 0.141984442865786
3.1 0.141984442865786
};
\addplot [line width=1pt, white, forget plot]
table {%
3.3 0.247618886526242
3.5 0.247618886526242
};
\addplot [line width=1pt, white, forget plot]
table {%
3.7 0.0878626303248753
3.9 0.0878626303248753
};
\addplot [line width=1pt, white, forget plot]
table {%
4.9 0.134968087815255
5.1 0.134968087815255
};
\addplot [line width=1pt, white, forget plot]
table {%
5.3 0.0402095843975281
5.5 0.0402095843975281
};
\addplot [line width=1pt, white, forget plot]
table {%
5.7 0.105071468625511
5.9 0.105071468625511
};
\end{axis}

\end{tikzpicture}


==> tex/velo_error_seq/velo_error_seq2.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{0.6,0,0.980392156862745}
% \definecolor{color1}{rgb}{0.968627450980392,0.00784313725490196,0.164705882352941}
% \definecolor{color2}{rgb}{0.0235294117647059,0.32156862745098,1}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
axis line style={white},
tick align=outside,
tick pos=left,
% title={Seq 2 },
x grid style={white!69.0196078431373!black},
xmin=0.5, xmax=6.3,
xtick style={color=black},
xtick={1.4,3.4,5.4},
xticklabels={X,Y,Z},
y grid style={white!69.0196078431373!black},
ylabel={Velocity Error (m/s)},
ymin=-0.0233556679147973, ymax=0.61,
ytick style={color=black},
    xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
]
\path [draw=color0, fill=color0]
(axis cs:0.9,0.0454993116751612)
--(axis cs:1.1,0.0454993116751612)
--(axis cs:1.1,0.149575866732583)
--(axis cs:0.9,0.149575866732583)
--(axis cs:0.9,0.0454993116751612)
--cycle;
\addplot [black, forget plot]
table {%
1 0.0454993116751612
1 0.000176190755700745
};
\addplot [black, forget plot]
table {%
1 0.149575866732583
1 0.298551854208258
};
\addplot [black, forget plot]
table {%
0.95 0.000176190755700745
1.05 0.000176190755700745
};
\addplot [black, forget plot]
table {%
0.95 0.298551854208258
1.05 0.298551854208258
};
\path [draw=color1, fill=color1]
(axis cs:1.3,0.0193088946071396)
--(axis cs:1.5,0.0193088946071396)
--(axis cs:1.5,0.0943910742063947)
--(axis cs:1.3,0.0943910742063947)
--(axis cs:1.3,0.0193088946071396)
--cycle;
\addplot [black, forget plot]
table {%
1.4 0.0193088946071396
1.4 0.000377116058847271
};
\addplot [black, forget plot]
table {%
1.4 0.0943910742063947
1.4 0.132937731845124
};
\addplot [black, forget plot]
table {%
1.35 0.000377116058847271
1.45 0.000377116058847271
};
\addplot [black, forget plot]
table {%
1.35 0.132937731845124
1.45 0.132937731845124
};
\path [draw=color2, fill=color2]
(axis cs:1.7,0.0512629607750226)
--(axis cs:1.9,0.0512629607750226)
--(axis cs:1.9,0.165225579088091)
--(axis cs:1.7,0.165225579088091)
--(axis cs:1.7,0.0512629607750226)
--cycle;
\addplot [black, forget plot]
table {%
1.8 0.0512629607750226
1.8 0.00075650953687223
};
\addplot [black, forget plot]
table {%
1.8 0.165225579088091
1.8 0.332121025821897
};
\addplot [black, forget plot]
table {%
1.75 0.00075650953687223
1.85 0.00075650953687223
};
\addplot [black, forget plot]
table {%
1.75 0.332121025821897
1.85 0.332121025821897
};
\path [draw=color0, fill=color0]
(axis cs:2.9,0.0417637473191679)
--(axis cs:3.1,0.0417637473191679)
--(axis cs:3.1,0.224785137712553)
--(axis cs:2.9,0.224785137712553)
--(axis cs:2.9,0.0417637473191679)
--cycle;
\addplot [black, forget plot]
table {%
3 0.0417637473191679
3 0.000264292467084815
};
\addplot [black, forget plot]
table {%
3 0.224785137712553
3 0.470813364165661
};
\addplot [black, forget plot]
table {%
2.95 0.000264292467084815
3.05 0.000264292467084815
};
\addplot [black, forget plot]
table {%
2.95 0.470813364165661
3.05 0.470813364165661
};
\path [draw=color1, fill=color1]
(axis cs:3.3,0.0448127976552481)
--(axis cs:3.5,0.0448127976552481)
--(axis cs:3.5,0.266378868864894)
--(axis cs:3.3,0.266378868864894)
--(axis cs:3.3,0.0448127976552481)
--cycle;
\addplot [black, forget plot]
table {%
3.4 0.0448127976552481
3.4 0.00411012798469557
};
\addplot [black, forget plot]
table {%
3.4 0.266378868864894
3.4 0.456005566679127
};
\addplot [black, forget plot]
table {%
3.35 0.00411012798469557
3.45 0.00411012798469557
};
\addplot [black, forget plot]
table {%
3.35 0.456005566679127
3.45 0.456005566679127
};
\path [draw=color2, fill=color2]
(axis cs:3.7,0.032206746853467)
--(axis cs:3.9,0.032206746853467)
--(axis cs:3.9,0.147270781441821)
--(axis cs:3.7,0.147270781441821)
--(axis cs:3.7,0.032206746853467)
--cycle;
\addplot [black, forget plot]
table {%
3.8 0.032206746853467
3.8 0.00140957279476162
};
\addplot [black, forget plot]
table {%
3.8 0.147270781441821
3.8 0.285432958940515
};
\addplot [black, forget plot]
table {%
3.75 0.00140957279476162
3.85 0.00140957279476162
};
\addplot [black, forget plot]
table {%
3.75 0.285432958940515
3.85 0.285432958940515
};
\path [draw=color0, fill=color0]
(axis cs:4.9,0.0365176475868445)
--(axis cs:5.1,0.0365176475868445)
--(axis cs:5.1,0.159425725571298)
--(axis cs:4.9,0.159425725571298)
--(axis cs:4.9,0.0365176475868445)
--cycle;
\addplot [black, forget plot]
table {%
5 0.0365176475868445
5 0.00350969869741924
};
\addplot [black, forget plot]
table {%
5 0.159425725571298
5 0.341189883516642
};
\addplot [black, forget plot]
table {%
4.95 0.00350969869741924
5.05 0.00350969869741924
};
\addplot [black, forget plot]
table {%
4.95 0.341189883516642
5.05 0.341189883516642
};
\path [draw=color1, fill=color1]
(axis cs:5.3,0.0352932972645825)
--(axis cs:5.5,0.0352932972645825)
--(axis cs:5.5,0.111943745306393)
--(axis cs:5.3,0.111943745306393)
--(axis cs:5.3,0.0352932972645825)
--cycle;
\addplot [black, forget plot]
table {%
5.4 0.0352932972645825
5.4 0.000227750891903522
};
\addplot [black, forget plot]
table {%
5.4 0.111943745306393
5.4 0.195521128516952
};
\addplot [black, forget plot]
table {%
5.35 0.000227750891903522
5.45 0.000227750891903522
};
\addplot [black, forget plot]
table {%
5.35 0.195521128516952
5.45 0.195521128516952
};
\path [draw=color2, fill=color2]
(axis cs:5.7,0.0305767420525668)
--(axis cs:5.9,0.0305767420525668)
--(axis cs:5.9,0.172522100116694)
--(axis cs:5.7,0.172522100116694)
--(axis cs:5.7,0.0305767420525668)
--cycle;
\addplot [black, forget plot]
table {%
5.8 0.0305767420525668
5.8 0.00128623420413865
};
\addplot [black, forget plot]
table {%
5.8 0.172522100116694
5.8 0.369336006006802
};
\addplot [black, forget plot]
table {%
5.75 0.00128623420413865
5.85 0.00128623420413865
};
\addplot [black, forget plot]
table {%
5.75 0.369336006006802
5.85 0.369336006006802
};
\addplot [line width=1pt, white, forget plot]
table {%
0.9 0.100766256788645
1.1 0.100766256788645
};
\addplot [line width=1pt, white, forget plot]
table {%
1.3 0.0682491611946423
1.5 0.0682491611946423
};
\addplot [line width=1pt, white, forget plot]
table {%
1.7 0.099464031339338
1.9 0.099464031339338
};
\addplot [line width=1pt, white, forget plot]
table {%
2.9 0.0989566119088892
3.1 0.0989566119088892
};
\addplot [line width=1pt, white, forget plot]
table {%
3.3 0.075984746026001
3.5 0.075984746026001
};
\addplot [line width=1pt, white, forget plot]
table {%
3.7 0.0908502564243308
3.9 0.0908502564243308
};
\addplot [line width=1pt, white, forget plot]
table {%
4.9 0.0821778973760645
5.1 0.0821778973760645
};
\addplot [line width=1pt, white, forget plot]
table {%
5.3 0.079976425217278
5.5 0.079976425217278
};
\addplot [line width=1pt, white, forget plot]
table {%
5.7 0.0728472717659245
5.9 0.0728472717659245
};
\end{axis}

\end{tikzpicture}


==> tex/velo_error_seq/velo_error_seq3.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{0.6,0,0.980392156862745}
% \definecolor{color1}{rgb}{0.968627450980392,0.00784313725490196,0.164705882352941}
% \definecolor{color2}{rgb}{0.0235294117647059,0.32156862745098,1}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
axis line style={white},
tick align=outside,
tick pos=left,
% title={Seq 3 },
x grid style={white!69.0196078431373!black},
xmin=0.5, xmax=6.3,
xtick style={color=black},
xtick={1.4,3.4,5.4},
xticklabels={X,Y,Z},
y grid style={white!69.0196078431373!black},
ylabel={Velocity Error (m/s)},
ymin=-0.0375045054404742, ymax=0.78781873238659,
ytick style={color=black},
    xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
]
\path [draw=color0, fill=color0]
(axis cs:0.9,0.050925850163972)
--(axis cs:1.1,0.050925850163972)
--(axis cs:1.1,0.305209551337428)
--(axis cs:0.9,0.305209551337428)
--(axis cs:0.9,0.050925850163972)
--cycle;
\addplot [black, forget plot]
table {%
1 0.050925850163972
1 0.000915280434687915
};
\addplot [black, forget plot]
table {%
1 0.305209551337428
1 0.658851716939473
};
\addplot [black, forget plot]
table {%
0.95 0.000915280434687915
1.05 0.000915280434687915
};
\addplot [black, forget plot]
table {%
0.95 0.658851716939473
1.05 0.658851716939473
};
\path [draw=color1, fill=color1]
(axis cs:1.3,0.0186842481424454)
--(axis cs:1.5,0.0186842481424454)
--(axis cs:1.5,0.103976060431693)
--(axis cs:1.3,0.103976060431693)
--(axis cs:1.3,0.0186842481424454)
--cycle;
\addplot [black, forget plot]
table {%
1.4 0.0186842481424454
1.4 0.000318754243475716
};
\addplot [black, forget plot]
table {%
1.4 0.103976060431693
1.4 0.180866270180915
};
\addplot [black, forget plot]
table {%
1.35 0.000318754243475716
1.45 0.000318754243475716
};
\addplot [black, forget plot]
table {%
1.35 0.180866270180915
1.45 0.180866270180915
};
\path [draw=color2, fill=color2]
(axis cs:1.7,0.0607938102103689)
--(axis cs:1.9,0.0607938102103689)
--(axis cs:1.9,0.255498452503433)
--(axis cs:1.7,0.255498452503433)
--(axis cs:1.7,0.0607938102103689)
--cycle;
\addplot [black, forget plot]
table {%
1.8 0.0607938102103689
1.8 0.000215207845459808
};
\addplot [black, forget plot]
table {%
1.8 0.255498452503433
1.8 0.509395351885571
};
\addplot [black, forget plot]
table {%
1.75 0.000215207845459808
1.85 0.000215207845459808
};
\addplot [black, forget plot]
table {%
1.75 0.509395351885571
1.85 0.509395351885571
};
\path [draw=color0, fill=color0]
(axis cs:2.9,0.0540813292258191)
--(axis cs:3.1,0.0540813292258191)
--(axis cs:3.1,0.234681439454613)
--(axis cs:2.9,0.234681439454613)
--(axis cs:2.9,0.0540813292258191)
--cycle;
\addplot [black, forget plot]
table {%
3 0.0540813292258191
3 0.00025457195519607
};
\addplot [black, forget plot]
table {%
3 0.234681439454613
3 0.50483313777927
};
\addplot [black, forget plot]
table {%
2.95 0.00025457195519607
3.05 0.00025457195519607
};
\addplot [black, forget plot]
table {%
2.95 0.50483313777927
3.05 0.50483313777927
};
\path [draw=color1, fill=color1]
(axis cs:3.3,0.0341207415404121)
--(axis cs:3.5,0.0341207415404121)
--(axis cs:3.5,0.341801049261369)
--(axis cs:3.3,0.341801049261369)
--(axis cs:3.3,0.0341207415404121)
--cycle;
\addplot [black, forget plot]
table {%
3.4 0.0341207415404121
3.4 0.00729099756574314
};
\addplot [black, forget plot]
table {%
3.4 0.341801049261369
3.4 0.750304039758087
};
\addplot [black, forget plot]
table {%
3.35 0.00729099756574314
3.45 0.00729099756574314
};
\addplot [black, forget plot]
table {%
3.35 0.750304039758087
3.45 0.750304039758087
};
\path [draw=color2, fill=color2]
(axis cs:3.7,0.0470434830938093)
--(axis cs:3.9,0.0470434830938093)
--(axis cs:3.9,0.190534730347155)
--(axis cs:3.7,0.190534730347155)
--(axis cs:3.7,0.0470434830938093)
--cycle;
\addplot [black, forget plot]
table {%
3.8 0.0470434830938093
3.8 0.000923772653984578
};
\addplot [black, forget plot]
table {%
3.8 0.190534730347155
3.8 0.397895565899473
};
\addplot [black, forget plot]
table {%
3.75 0.000923772653984578
3.85 0.000923772653984578
};
\addplot [black, forget plot]
table {%
3.75 0.397895565899473
3.85 0.397895565899473
};
\path [draw=color0, fill=color0]
(axis cs:4.9,0.0370850724055838)
--(axis cs:5.1,0.0370850724055838)
--(axis cs:5.1,0.144242538996679)
--(axis cs:4.9,0.144242538996679)
--(axis cs:4.9,0.0370850724055838)
--cycle;
\addplot [black, forget plot]
table {%
5 0.0370850724055838
5 1.01871880286986e-05
};
\addplot [black, forget plot]
table {%
5 0.144242538996679
5 0.29127738534024
};
\addplot [black, forget plot]
table {%
4.95 1.01871880286986e-05
5.05 1.01871880286986e-05
};
\addplot [black, forget plot]
table {%
4.95 0.29127738534024
5.05 0.29127738534024
};
\path [draw=color1, fill=color1]
(axis cs:5.3,0.0345189067087442)
--(axis cs:5.5,0.0345189067087442)
--(axis cs:5.5,0.216801981745139)
--(axis cs:5.3,0.216801981745139)
--(axis cs:5.3,0.0345189067087442)
--cycle;
\addplot [black, forget plot]
table {%
5.4 0.0345189067087442
5.4 0.00468124038173312
};
\addplot [black, forget plot]
table {%
5.4 0.216801981745139
5.4 0.421482532405152
};
\addplot [black, forget plot]
table {%
5.35 0.00468124038173312
5.45 0.00468124038173312
};
\addplot [black, forget plot]
table {%
5.35 0.421482532405152
5.45 0.421482532405152
};
\path [draw=color2, fill=color2]
(axis cs:5.7,0.0333654972375574)
--(axis cs:5.9,0.0333654972375574)
--(axis cs:5.9,0.145628655344953)
--(axis cs:5.7,0.145628655344953)
--(axis cs:5.7,0.0333654972375574)
--cycle;
\addplot [black, forget plot]
table {%
5.8 0.0333654972375574
5.8 0.000549304948028739
};
\addplot [black, forget plot]
table {%
5.8 0.145628655344953
5.8 0.312894917001754
};
\addplot [black, forget plot]
table {%
5.75 0.000549304948028739
5.85 0.000549304948028739
};
\addplot [black, forget plot]
table {%
5.75 0.312894917001754
5.85 0.312894917001754
};
\addplot [line width=1pt, white, forget plot]
table {%
0.9 0.129738371745527
1.1 0.129738371745527
};
\addplot [line width=1pt, white, forget plot]
table {%
1.3 0.0536968219671419
1.5 0.0536968219671419
};
\addplot [line width=1pt, white, forget plot]
table {%
1.7 0.107509878653638
1.9 0.107509878653638
};
\addplot [line width=1pt, white, forget plot]
table {%
2.9 0.121060592272317
3.1 0.121060592272317
};
\addplot [line width=1pt, white, forget plot]
table {%
3.3 0.109664642493887
3.5 0.109664642493887
};
\addplot [line width=1pt, white, forget plot]
table {%
3.7 0.119131419941609
3.9 0.119131419941609
};
\addplot [line width=1pt, white, forget plot]
table {%
4.9 0.0768678127111805
5.1 0.0768678127111805
};
\addplot [line width=1pt, white, forget plot]
table {%
5.3 0.115904482344118
5.5 0.115904482344118
};
\addplot [line width=1pt, white, forget plot]
table {%
5.7 0.083997795576003
5.9 0.083997795576003
};
\end{axis}

\end{tikzpicture}

